Collaborative Learning in Kernel-based Bandits for Distributed Users

We study collaborative learning among distributed clients facilitated by a central server. Each client is interested in maximizing a personalized objective function that is a weighted sum of its local objective and a global objective. Each client has direct access to random bandit feedback on its local objective, but only has a partial view of the global objective and relies on information exchange with other clients for collaborative learning. We adopt the kernel-based bandit framework where the objective functions belong to a reproducing kernel Hilbert space. We propose an algorithm based on surrogate Gaussian process (GP) models and establish its order-optimal regret performance (up to polylogarithmic factors). We also show that the sparse approximations of the GP models can be employed to reduce the communication overhead across clients.

==> arXiV version copy/Algorithm.tex <==
\section{The CEPE Policy}
\label{section:policy}

In this section, we describe our proposed algorithm for the problem of personalized kernel bandits.

\subsection{Algorithm Description}\label{sec:flex_description}

The design of a collaborative learning policy such as CEPE significantly deviates from those for single client settings. If one were to design a collaborative learning algorithm by simply deploying a classical centralized kernel-based learning algorithm like GP-UCB or GP-TS~\cite{Chowdhury2017} at each client to learn their personalized rewards, then such an algorithm could result in a trivial regret, linearly growing with $T$. This can be attributed to the fact that the personalized objective function $f_i$ of client $i$ contains the local observation functions $\{h_j\}_{j\neq i}$ of other clients that are not observable to client $i$. If client $i$ were to use GP-UCB on their personalized reward, then their query points would quickly concentrate around $x_i^*$ making it difficult for a client $j$ to satisfactorily learn $h_i$ (and hence $f_j$) especially in regions far away from $x_i^*$,  even if all the observations of client $i$ were available to client $j$. Hence, Collaborative Exploration is necessary for each client to learn the maximizer $x_i^*$ of its personalized objective function $f_i$.
% For example, consider two clients with significantly different optimum points $x_1^*\neq x_2^*$, $f_1(x_1^*)\gg f_1(x_2^*)$ and $f_2(x_2^*)\gg f_2(x_1^*)$. Then, using an algorithm with low regret in the single client setting (e.g., GP-UCB or GP-TS), the observations of client $1$ should ideally concentrate around $x_1^*$, meaning client $1$ does not provide informative observations about $h_1(x_2^*)$ to client $2$. Those, however, are crucial for client $2$ being able to get closer to $x_2^*$. The same is true about the crucial information which client $1$ requires from client $2$. Thus, in a collaborative learning algorithm, it is necessary for each client to provide altruistic observations for others to allow all clients to learn their own maximum personalized reward. 
This adds another layer of nuance to the exploration-exploitation trade-off as the exploration at any client needs to serve the goal of greater good instead of being sufficient for local exploitation.  \\

Inspired by \emph{deterministic sequencing of exploration and exploitation (DSEE)} algorithm for discrete bandits for centralized learning~\cite{Vakili2013}, we propose CEPE, a kernel-based collaborative learning policy that effectively trades off exploration and exploitation in a distributed learning setting. We first describe the design of the interleaving exploration and exploitation epochs, a central component in CEPE. Following that, we describe the communication protocol and the query policy adopted in CEPE that ensures a low communication cost along with an overall low regret.
  





% In this section, we present the FLEX policy. The policy consists of interleaving exploration and exploitation sequences. In the exploration sequence, all the clients contribute to learning the local observation functions $g_i$, by choosing observation points distributed across the entire domain. This is crucial for all the clients to learn their own personalized reward functions. In the exploitation sequence, the clients aim at achieving maximum possible personalized reward, based on the information gathered so far. The cardinality of the exploration sequence is carefully designed in a way to optimally trade off the exploration and exploitation, and guarantee low regret. In addition, the separation between exploration and exploitation allows effective control of information exchange across clients for learning the global objective. Both exploration and exploitation in FLEX policy are guided by a fictitious Gaussian process (GP) prior for the elements of the RKHS. We refer to the GP model as fictitious to signify that the use of GP model is only for policy design and does not affect our regularity assumptions given in Section~\ref{sec:problem_formulation}. 
% Before presenting FLEX, we overview the GP models and some useful confidence intervals for the RKHS elements based on GP models, which are central to our policy design. 

\subsubsection{The interleaving epoch structure}

CEPE divides the time horizon of $T$ steps into interleaving epochs of exploration and exploitation of increasing lengths. The length of each epoch is fixed at the beginning of the algorithm based on $N_t:\N\rightarrow \R$, a positive non-decreasing sequence of real numbers that is assumed to have been provided as an input to CEPE. Let $\cA(t)$ denote the collection of time instants at which CEPE had carried out an exploration step up to time $t -1$. CEPE decides to explore at a time instant $t$ if $|\cA(t)| \leq N_t$, otherwise it decides to exploit at time $t$. As a concrete example, consider the case where $N_t = t^{2/3}$ for $t \in N$. At $t = 1$, $|\cA(1)| = 0$ as no point has been explored before it. Since $N_1 = 1 > |\cA(1)|$, CEPE explores at $t = 1$. For $t = 2$, evidently $|\cA(2)| = 1$ and $N_2 = 2^{2/3} > 1$ implying CEPE again explores at $t = 2$. Similarly, CEPE also explores at $t = 3$ as $|\cA(3)| = 2 < N_3$. However, at $t = 4$, $|\cA(4)| = 3$ while $N_4 < 3$. Consequently, CEPE begins an exploitative epoch at $t = 4$ and extends to $t = 5$ as $|\cA(5)| = 3 > N_5$. Once again at $t = 6$, $|\cA(6)| < N_6$ and CEPE decides to explore, terminating the first exploitative epoch and beginning the second exploratory epoch. This process repeats until the end of the time horizon.   \\

The design of the exploration-exploitation epochs is a central piece of the puzzle as it is related to both the communication cost and the regret due to its implicit links with the communication protocol of CEPE and the design of the update rule of the decision rule, as described below.

\subsubsection{Communication Protocol}

CEPE adopts a straightforward, easy to implement communication and message exchange protocol. All the communication between the clients and the server happens only during an exploration epoch. CEPE forgoes communication during exploitation epoch to ensure a low communication overhead. Thus, the separation between exploration and exploitation allows effective control of information exchange across clients for learning the global objective while simultaneously helping limit the communication overhead. \\

At every time instant $t$ during an exploration epoch, each client sends the value of the current decision variable queried, $x_{i ,t}$ along with the observed random reward, $y_{i,t}$ to the server. The server then broadcasts this to all clients. \\


% While the decision to communicate is the same, the message exchange protocol is slightly different in the two different use cases. In the setup of clients with access to compute power,  For applications with low-cost dispensable users, the server first sends the $x_{i,t}$ to the client and the client only sends back the observed random reward, $y_{i,t}$ for all time $t$ in any exploration epoch. Additionally, the server sends each client the point to be queried during an exploitation epoch, once at the beginning of the epoch. In the setup, since the server is carrying out all the computation, it obviates the broadcast step.

We would like to point out that such a communication scheme does not violate any privacy concerns and is designed in a similar spirit to various distributed learning algorithms, especially in the scenario of Federated Learning. Similar to any FL algorithm, CEPE only communicates the current model parameters (the decision variable $x$ in this setup) and not the actual data. The only difference is that CEPE also communicates a random loss associated with the current decision variable, which also does not give access to any actual data held by the clients. Thus, CEPE also ensures privacy by avoiding data sharing as considered in FL setups.


\subsubsection{Query Policy}

The only step left to specify is the update rule of decision variable, $x$, used in CEPE. The update rule is based on whether the current time instant belongs to an explorative or an exploitative epoch and is guided by a fictitious Gaussian process (GP) prior for the elements of the RKHS, as described in Section~\ref{sec:GP}. During an exploratory epoch, the clients choose different points across the epoch for continual learning. In particular, client $i$ chooses $x_{i,t} = \argmax_{x \in \cX} \sigma_{t-1}^{(h_i)}(x)$, where $\sigma_{t-1}^{(h_i)}(\cdot)$ is the posterior standard deviation of the GP model of $h_i$ based on all the previous exploratory observations $\cS_{i,t} = \{ (x_{i,s}, y_{i,s}) : s \in \cA(t) \}$ of client $i$ according to equation~\eqref{eq:posterior_variance}. On the other hand, during an exploitation epoch the query point is fixed and chosen to maximize earning and forgo learning. Specifically, each client $i$ chooses a point with the highest predicted value based on the GP model, i.e., $x_{i,t} = \argmax_{x\in\cX} \mu_{t-1}^{(f_i)}(x),$ where $\mu_{t-1}^{(f_i)}(\cdot)$ is the posterior mean of the personalized reward function, given as
\begin{align*}
    \mu_{t-1}^{(f_i)}(\cdot) = \alpha_i \mu_{t-1}^{(h_i)}(\cdot) + \frac{(1 - \alpha_i)}{K} \sum_{j = 1}^K \mu_{t-1}^{(h_j)}(\cdot).
\end{align*}
In the above expression $\mu_{t-1}^{(h_j)}(\cdot)$ are the posterior means of the GP model of $h_j$ based on all the previous exploratory observations $\cS_{j,t}$ corresponding to client $j = 1, 2, \dots, K$. We also provide a pseudocode in Alg.~\ref{alg:fed_exp_2} that succinctly combines the three design components of CEPE. 


\begin{algorithm}
	\caption{Collaborative Exploration with Personalized Exploitation (CEPE)}
	\label{alg:fed_exp_2}
	\begin{algorithmic}
		\STATE {\bfseries Input:} $\{B_j\}_{j = 1}^{K}$, the kernel $k(\cdot, \cdot)$, $\{N_t\}_{t \in \N}$
		\STATE Set $t \leftarrow 1$, $\cA(1) \leftarrow \emptyset$
	    \REPEAT
	    \IF{$|\cA(t)| < N_t$} 
	    \STATE $\cA(t + 1) = \cA(t) \cup \{t\}$
	    \ENDIF
	    \IF{$t \in \cA(t + 1)$}
	    \STATE $x_{i,t} = \argmax_{x \in \cX} \sigma_{t-1}^{(h_i)}(x)$
	    \ELSE
	    \STATE $x_{i,t} = \argmax_{x\in\cX} \mu_{t-1}^{(f_i)}(x)$
	    \ENDIF
	    \STATE Query the function $h_i$ at $x_{i,t}$ to obtain $y_{i,t}$
	    \IF{$t \in \cA(t+1)$}
	    \STATE Send $(x_{i,t}, y_{i,t})$ to the server which is then broadcast to all clients 
	    \ENDIF
            \STATE $t \leftarrow t + 1$
	    \UNTIL{$t = T$}
	\end{algorithmic}
\end{algorithm}


\subsection{Performance Analysis}


The theorem below establishes an upper bound on the regret performance of CEPE.

\begin{theorem}
Consider the kernel-based collaborative learning with personalized rewards setting described in Section~\ref{sub:fl_personalization}. Under Assumptions~\ref{assumption1} and~\ref{assumption:sub_gaussian} and for a given sequence $\{N_t\}_{t \in \N}$, the regret performance of CEPE satisfies, for any $\delta_0 \in (0,1)$, with probability at least $1-\delta_0$, 
\begin{eqnarray}
R_{\text{CEPE}}(T) =\cO\left(
K N_T + K T\sqrt{\frac{\gamma_{N_T}}{N_T} \log \left( \frac{T}{\delta_0}  \right)} \nonumber
\right)
\end{eqnarray}
In particular, the regret is minimized with the choice of $N_T=\Theta(T^{\frac{2}{3-\kappa}}(\log(T/\delta_0))^{\frac{1}{3}})$ in which case,
\begin{align*}
    R_{\text{CEPE}}(T) =\cO(KT^{\frac{2}{3 - \kappa}}(\log({T/\delta_0}))^{\frac{1}{3}} ). \nonumber
\end{align*}
% \begin{eqnarray}
% R_{\text{CEPE}}(T) =\Oc(KT^{2/3}(\gamma_T\log({1/\delta_0}))^{1/3} ). \nonumber
% \end{eqnarray}
\label{thm:regret_fed_exp}
\end{theorem}
Recall that $\gamma_t = \Oc(t^{\kappa})$ with $\kappa \in (0,1]$ corresponds to the maximal information gain of the kernel $k$. Specifically, if the underlying kernel is a Matern kernel with smoothness parameter $\nu$, then it is known that $\kappa = d/(2\nu + d)$~\cite{Vakili2020infogain}. Consequently, the regret incurred by CEPE is given as $\cO(T^{\frac{2\nu + d}{3\nu  + d}})$. In the case of a Squared Exponential kernel, $\kappa \to 0$ and hence $R_{\text{CEPE}}(T) = \cO(T^{2/3} (\log (T))^{d/6})$. \\



% In Theorem~\ref{thm:regret_fed_exp}, $\gamma_t$ is the maximal information gain, and is representative of the effective dimension of the kernel. It is defined as $\gamma_t := \max_{A \subset {\cX}: |A| = t} I(y_A; h_A)$ where, $I(y_A; h_A)$ denotes the mutual information between $h_A = [h(x)]_{x \in A}$ and $y_A = h_A + \epsilon_A$. Bounds on $\gamma_t$ for several common kernels are known~\cite{Srinivas2012, Vakili2020infogain} and are increasing sublinear functions of $t$. 

\begin{proof}
We here provide a sketch of the proof. We bound the regret in the exploration and exploitation epochs separately. The bound on the RKHS norm of $f_i$ implies a bound on its sup norm. Thus, the regret in the exploration epoch is simply bounded by $\Oc(KN_T)$. The regret during the exploitation epoch is bounded using Lemma~\ref{lemma:concentration_bound} based on the posterior variance of the GP model. Maximal uncertainty reduction sampling and a known bound on the total uncertainty (cumulative conditional variances) of a GP model based on information gain allows us to bound the posterior variance with an $\Oc(\frac{\gamma_{N_t}}{N_t})$ term. Combining these two results, we bound the regret in the exploitation epoch. A detailed proof of Theorem~\ref{thm:regret_fed_exp} is provided in Appendix~\ref{proof:regret_fed_exp}.
\end{proof}


% We here provide a sketch of the proof. We bound the regret in the exploration and exploitation epochs separately. The bound on the RKHS norm of $f_i$ implies a bound on its sup norm. Thus, the regret in the exploration epoch is simply bounded by $\Oc(KN_T)$. The regret during the exploitation epoch is bounded using Lemma~\ref{lemma:concentration_bound} based on the posterior variance of the GP model. Maximal uncertainty reduction sampling and a known bound on the total uncertainty (cumulative conditional variances) of a GP model based on information gain allows us to bound the posterior variance with an $\Oc(\frac{\gamma_{N_t}}{N_t})$ term. Combining these two results, we bound the regret in the exploitation epoch. A detailed proof of Theorem~\ref{thm:regret_fed_exp} is provided in~\cite{SalgiaPersonalization2022} 
% \blue{and the supplementary material (I think TSP allows supplementary material; it is better to submit the proofs as supplementary material as well if they do not fit into the page limit.)}. 
% the supplementary material . %Appendix~\ref{proof:regret_fed_exp}.



% We here provide a sketch of the proof of the theorem. To bound the regret of PerK, the regret incurred during the exploration and exploitation sequences is considered separately. For the points in the exploration sequence, we bound $f(x_{i}^*) - f(x_{i,t})$ trivially by $2B_i$ for every client which when summed yields the $\Oc(KN_T)$ term. For the points in the exploitation sequence, we use Lemma~\ref{lemma:concentration_bound} to bound $|f_i(x_i^*) - f(x_{i,t})|$ in terms of the posterior standard deviation at $x_i^*$ and $x_{i,t}$. Using the properties of the maximum posterior variance sampling scheme, we bound the posterior standard deviation at $x_i^*$ and $x_{i,t}$ by $\Oc(\sqrt{\gamma_{N_t}/N_t})$ which on summing yields the second term in the expression. A detailed proof of the Theorem is provided in Appendix~\ref{proof:regret_fed_exp}.


\begin{remark}\label{remark:singlekernel}
The upper bound on the regret of CEPE given in Theorem~\ref{thm:regret_fed_exp} is sublinear in $T$ as $\gamma_T=o(T)$ for typical kernels~\cite{Vakili2020infogain}. A sublinear regret bound guarantees the convergence to the maximum personalized reward $f_i(x_i^*)$ across all clients, as $T$ grows. We would like to emphasize the significance of this guarantee for the performance of CEPE. In comparison, it is not clear whether standard algorithms such as GP-UCB or GP-TS achieve sublinear regret, even in the simpler problem of a single client. The existing upper bounds on the regret performance of these algorithms are in the form of $\tilde{\mathcal{O}}(\gamma_T\sqrt{T})$, which may be trivial, as $\gamma_T$ may grow faster that $\sqrt{T}$. For example, that is the case with a broad range of parameters in the case of Mat{\'e}rn kernel (see~\cite{vakili2021open} for a detailed discussion). The CEPE algorithm thus may be of interest even for a single client setting, in terms of introducing a simple algorithm with sublinear regret. We, however, note that more sophisticated algorithms such as GP-ThreDS~\cite{Salgia2020GPThreDS}, SupKernelUCB~\cite{Valko2013a}, and BPE~\cite{li2022gaussian} achieve better regret bounds in the case of a single client.
% GP-ThreDS is based on domain-shrinking methodology and forming a random walk on a tree representing the sub-domain structure. SupKernelUCB builds on episodic independent batches of observations; it however has been shown to perform poorly in practice~\cite{Cai2020, Calandriello2019}.
\end{remark}

% \vspace{-1em}
% \paragraph{Choosing the exploration sequence:}
% A key design parameter in CEPE is the size $N_T$ of the exploration sequence. It determines the performance of the algorithm by controlling the trade-off between the cost of exploration and the cost of exploitation. This is seen in the expression of regret given in Theorem~\ref{thm:regret_fed_exp}. The first term, $\mathcal{O}(KN_T)$, corresponds to the regret incurred during the exploration sequence, and increases with $N_T$. The second term, $\mathcal{O}\left(KT\sqrt{\frac{\gamma_{N_T}}{N_T}\log(\frac{1}{\delta_0})}\right)$, corresponds to the regret incurred during exploitation, and decreases with $N_T$. That is, a larger exploration sequence enables a better approximation of the arm statistics, which leads to a better performance during the exploitation sequence. The optimal size $N_T$ of the exploration sequence is one that minimizes the larger value between these two terms. That is how $N_T=\Theta(T^{2/3}(\gamma_T\log(1/\delta_0))^{1/3})$ in Theorem~\ref{thm:regret_fed_exp} is selected. 

We would like to emphasize the role of the sequence $\{N_t\}_{t \in \N}$ in the context of the performance of CEPE, both in terms of regret and communication cost. It affects both these metrics through the overall amount of exploration carried out in CEPE. In particular, at the end of the time horizon, CEPE would have explored for no more than $N_{T}$ time steps. The impact of this on the regret can be noted from the statement of Theorem~\ref{thm:regret_fed_exp}. The first term, $\mathcal{O}(KN_T)$, corresponds to the regret incurred during the exploration sequence, and increases with $N_T$. The second term, $\mathcal{O}\left(KT\sqrt{\frac{\gamma_{N_T}}{N_T}\log(\frac{1}{\delta_0})}\right)$, corresponds to the regret incurred during exploitation, and decreases with $N_T$. That is, a larger exploration sequence enables a better approximation of the arm statistics, which leads to a better performance during the exploitation sequence. On the other hand, since CEPE communicates at all and only the exploration time instants, its communication cost is bounded by $N_{T}$. Thus, CEPE controls the communication-regret trade-off through this sequence $N_t$ and one can appropriately choose the sequence to trade-off the regret against communication based on the demands of a particular application. For example, if the objective is to minimize regret, then the optimal size $N_T$ is obtained by minimizing the larger of the two terms in expression of regret, yielding us $N_T=\Theta(T^{\frac{2}{3- \kappa}}(\log(1/\delta_0))^{\frac{1}{3}})$, as referred to in Theorem~\ref{thm:regret_fed_exp}. Under this scenario, CEPE incurs a communication cost of $\cO(T^{2/(3- \kappa)})$, which is sublinear in $T$.











% \subsection{PerK}\label{sec:policyPerK}

% There exist several kernel-based learning algorithms including GP-UCB and GP-TS~\cite{Chowdhury2017} for a single client setting. We note that even if all the observations of each client were available to all other clients, following the existing algorithms on personalized rewards would result in a trivial regret, linearly growing with $T$. For example, consider two clients with significantly different optimum points $x_1^*\neq x_2^*$, $f_1(x_1^*)\gg f_1(x_2^*)$ and $f_2(x_2^*)\gg f_2(x_1^*)$. Then, using an algorithm with low regret in the single client setting (e.g., GP-UCB or GP-TS), the observations of client $1$ should ideally concentrate around $x_1^*$, meaning client $1$ does not provide informative observations about $g_1(x_2^*)$ to client $2$. Those, however, are crucial for client $2$ being able to get closer to $x_2^*$. The same is true about the crucial information which client $1$ requires from client $2$. We thus need to design a collaborative algorithm where each client provides altruistic observations for others, which will eventually be beneficial for all the clients, and allow them to learn their own maximum personalized reward.   



% We first describe the design of exploration-exploitation sequences in PerK followed by the messaging passing protocol and the update rule for the decision variables as the last step.
% . The selected points in each sequence are guided based on the statistics provided by the GP model.  %fictitious
% \emph{Designing the exploration-exploitation sequences}: 


% While we specify the exact rule adopted by PerK in the third step, the high-level design objective is to linked to the nature of epoch as follows. During an exploratory epoch, the clients choose different points across the epoch for continual learning. On the other hand, the decision variable during an exploitation variable should be fixed and chosen to maximize earning and forgo learning.











% Here you only present the high-level design objective: x_t chosen to explore during exploration epochs and changes at each time step for continual learning; x_t chosen to exploit during exploitation epochs and fixed within an exploitation epochs (earning and no learning to reduce message exchange)  
% Message exchange: specify the two ways of exchange (when and what to be exchanged, who is doing the computation).

% Having assigned each time instant to a exploratory or exploitative epoch, the choice of the decision variable at a time $t$, i.e., $x_t$, is determined by the corresponding epoch.

% point to be queried at that instant is determined by the corresponding epoch. In particular, during an exploratory epoch, each client chooses different points to explore their local observation function while in an exploitative epoch, each client plays a single action throughout the epoch to maximize their reward.


% the exploration sequence up to time $t$, meaning if $s\in\cA(t)$, the clients explore at time $s$, then 





% Let $\cA(t)$ denote the exploration sequence up to time $t$, meaning if $s\in\cA(t)$, the clients explore at time $s$. The exploration in PerK is designed to maximally reduce the uncertainty about the local observation functions $g_i$, using the variance (uncertainty estimate) provided by the fictitious GP model. In particular, when $t\in\cA(t)$, client $i$ chooses
% \[
% x_{i,t} = \argmax_{x \in \cX} \sigma_{t-1}^{(g_i)}(x),
% \]
% where $\sigma_{t-1}^{(g_i)}(\cdot)$ is the posterior standard deviation of the GP model of $g_i$ based on all the previous exploratory observations $\cS_{i,t} = \{ (x_{i,s}, y_{i,s}) : s \in \cA(t-1) \}$ of client $i$ according to equation~\eqref{eq:posterior_variance}.

% In the exploitation sequence, each client $i$ chooses a point with the highest predicted value based on the GP model. In particular, when
% $t\not\in\cA(t)$, client $i$ chooses
% \[
% x_{i,t} = \argmax_{x\in\cX} \mu_{t-1}^{(f_i)}(x),
% \]
% where $\mu_{t-1}^{(f_i)}(\cdot)$ is the posterior mean of the personalized reward function, given as
% \begin{align*}
%     \mu_{t-1}^{(f_i)}(\cdot) = \alpha_i \mu_{t-1}^{(g_i)}(\cdot) + \frac{(1 - \alpha_i)}{K} \sum_{j = 1}^K \mu_{t-1}^{(g_j)}(\cdot).
% \end{align*}
% In the above expression $\mu_{t-1}^{(g_j)}(\cdot)$ are the posterior mean of the GP model of $g_j$ based on all the previous exploratory observations $\cS_{j,t}$ corresponding to client $j = 1, 2, \dots, K$.

%  = \{ (x_{j,s}, y_{j,s}) : s \in \cA(t-1) \}

% based on all the previous observations $\cS_t(j) = \{ (x_s^{(j)}, y_s^{(j)}) : s \in \cA(t-1) \}$. The posterior mean for $f_i$, $\mu_{i, t-1}^{f_i}(\cdot)$, is given  


% \emph{Communication:} The observations $\cS_{i,t}$ of each client $i$ in the exploration sequence  are communicated to the server which is then broadcast to all other clients. An advantage of PerK is that the amount of communication can be easily controlled by the cardinality of the exploration sequence. 

% \emph{The cardinality of the exploration sequence:} We define the exploration sequence as follows: if $|\cA(t)| < N_t$, then $\cA(t + 1) = \cA(t) \cup \{t + 1\}$, where $N_t:\N\rightarrow \R$ is a positive non-decreasing sequence of real numbers, controlling the cardinality of the exploration sequence.


% \emph{The cardinality of the exploration sequence:} We define the exploration sequence as follows: if $|\cA(t)| < C (t+1)^{\theta}$, then $\cA(t + 1) = \cA(t) \cup \{t + 1\}$, for some $\theta\in[0,1]$. 

% The conventional approach in kernelized bandit settings is to use the Upper Confidence Bound (UCB) score to build a proxy of the function which is then maximized to obtain the next query point. The UCB score tacitly captures the bias-variance tradeoff in estimating the function. As a result, policies that employ the UCB score address the exploration-exploitation trade-off implicitly while maximizing the UCB. Unlike the single agent case, in this setting of federated bandits with personalization involving multiple agents, it is necessary for learning policies to have explicit exploration sequences to achieve sublinear regret guarantees. This can be attributed to the fact that exploitation and exploration are not tailored to the same function. Specifically, in the single agent case, there is only function that needs to be explored or exploited. On the other hand, in this multi-agent case, each agent is interested in exploiting their own objective function near its maximum value but at the same time has to explore their local functions over the entire domain to help get better estimates of the global reward function. The key to address this pronounced trade-off lies in developing learning policies that incorporate a component of ``social welfare'', reminiscient of cooperative strategies in Game Theory literature. 

% The proposed policy, PerK, is thus designed to achieve a sublinear regret by replacing selfish actions of the agents in the that exploit their own objective functions by exploration sequences designed to benefit the set of agents a whole and in particular the individual agents by helping them learn the global reward function and consequently their objective function better. Specifically, FLEX divides the entire time horizon into two interleaving sequences -- an exploration and an exploitation sequence, similar to MAB algorithm in~\cite{}. In the exploration sequence, the agents are directed to query those points that contribute towards getting a better idea of the landscape of their local reward function instead of minimizing regret. In terms of the kernelized bandit setup, FLEX implements this by directing agents to query points with maximum posterior variance helping reduce the overall uncertainty in estimating the local reward functions. In the exploitation sequence, the agents simply choose the maximizer of UCB of their objective function. In this step, we construct the UCB score based on the posterior mean and variance computed using only the samples obtained during the exploration sequence. This is in contrast with the standard approaches where the entire history is used to obtaining the posterior mean and variance. We show that such a choice is not only sufficient to obtain optimal regret but also reduces the computational burden as the total length of the exploration sequence is sublinear in the time horizon. A detailed implementation of the algorithm for agent $i$ is provided in~\ref{}. 

% In the pseudo-code outlined in Alg.~\ref{}, $\mu_{t-1}^{(j)}$ and $\sigma_{t-1}^{(j)}$ denote the posterior mean and standard deviation obtained from the GP model for the local reward function of agent $j$
% at the points sampled by agent $j$ until time $t$ given by $\cS_t(j) = \{ (x_s^{(j)}, y_s^{(j)}) : s \in \cA(t-1) \}$.


% $U_{t-1}^{(i)}$ denotes the upper confidence bound of the objective function of agent $i$ at time $t$ and is given as
% \begin{align*}
%     U_{t-1}^{(i)} & = \alpha_i(\mu_{t-1}^{(i)} + \beta_i (\delta) \sigma_{t-1}^{(i)}) + \\
%     & \ \ \ \ \ \ \ \frac{1 -\alpha_i}{K} \sum_{j=1}^K (\mu_{t-1}^{(j)} + \beta_j (\delta) \sigma_{t-1}^{(j)}).
% \end{align*}
% Here $\mu_{t-1}^{(j)}$ and $\sigma_{t-1}^{(j)}$ denote the posterior mean and standard deviation obtained from the GP model for the local reward function of agent $j$
% at the points sampled by agent $j$ until time $t$ given by $\cS_t(j) = \{ (x_s^{(j)}, y_s^{(j)}) : s \in \cA(t-1) \}$. Agent $i$ has access to this posterior mean and variance as all the observations taken during the exploration period by any agent are broadcast to everyone. Lastly, $\beta_j(\delta) = B_j + R\sqrt{\log(1/\delta)/\lambda}$ where recall that $R$ is the sub-Gaussian proxy variance and $\lambda$ is the variance of the Gaussian noise model.

% Moreover, such a cooperative behaviour is actually necessitated by the need for personalization. In fact, it is possible to come up with policies that do not need such cooperative behaviour when operating at the either end of the spectrum, that is, a local model or a completely global model.

% Referred to as ``GP-UCB-DSEE" \textcolor{red}{(can change this later)}, the proposed algorithm consists of a sequence of interleaved exploration and exploitation sequences of a pre-determined length similar to the DSEE algorithm for multi-armed bandits. Such an interleaved exploration-exploitation sequence is in contrast with the standard approaches used in kernelized bandit settings. 

% Our proposed policy, also 



% An important aspect of FLEX is the parameter $\theta$ that determines the length of the exploration sequence. This parameter allows us to tradeoff communication cost with regret. In particular, since only the points in the exploration sequence are communicated to the central server, the communication cost of any agent is equal to the length of the exploration sequence as each such transmission has a unit cost. It can be shown that for $\theta \in (0, \theta_0]$, regret decreases as $\theta$, or equivalently the length of exploration sequence, increases. Consequently, it is possible to decrease the regret at the cost of increased communication. The decrease in regret can be attributed to the better estimates of the global reward attained for longer exploration sequences. On increasing $\theta$ beyond $\theta_0$, both regret and communication cost increase, indicating that it is always sub-optimal to operate in that regime of $\theta$. In fact, as shown in the theorem below, the regret is indeed minimized for $\theta = \theta_0$. Consequently, FLEX has an inbuilt parameter to trade-off communication cost with regret performance that can be tuned according to the specifications of the particular application or setup.




% Thus, we would like to make this term as small as possible. On the other hand, an under exploration, caused by setting $N_T$ too small, leads to poor estimation of the arm statistics, and consequently a high regret during the exploitation sequence. That corresponds to the second term~$\mathcal{O}(KT\sqrt{\frac{\gamma_{N_T}}{N_T}\log(\frac{1}{\delta_0})})$ in the regret expression in Theorem~\ref{thm:regret_fed_exp}. The optimal value of $N_T$ is obtained as the value that minimizes the larger term between these two terms. On minimizing $\max\{N_T, T\sqrt{\gamma_T/N_T}\}$, we obtain that the optimal value of $N_T$ is $N_T=\Theta(T^{\frac{2}{3}}(\gamma_T\log(1/\delta_0))^{\frac{1}{3}})$.






% GP-ThreDS is based on methodology of domain-shrinking where the sub-domain structure is traversed using a random walk.


% \begin{theorem}
% Consider the kernel based FL with personalization setting described in Sec~\ref{}. If FLEX is applied to this setup for a given value of $\theta$, then the regret incurred by it satisfies $O(T^{\theta} + T^{1 - \theta/2}\gamma_T^{\theta/2})$. Moreover, if $\gamma_T = \Theta(T^{\nu})$, then the regret is minimized for $\theta = 2/(3 - \nu)$ and the corresponding minimum value is $O(T^{2/(3-\nu)})$.
% \end{theorem}

% From the above theorem, one can note that the regret as $\theta$ increases until $\theta = 2/(3 - \nu)$ after which the regret begins to increase with $\theta$, as mentioned earlier. In practice, it might be easier to set $\theta$ to $2/3$, a kernel agnostic choice. In such a case, the regret incurred by the algorithm is $O(T^{2/3} \gamma_T^{1/3})$ which is only marginally larger than the optimal value and always guaranteed to be sublinear.

% \emph{Proof Sketch.} To bound the regret of FLEX, we consider the regret incurred during the exploration and exploitation sequences separately. The regret corresponding to the exploration sequence is bounded with a constant factor of the cardinality of the exploration sequence, yielding the $K N_T$ term. The bound on the regret corresponding to the exploitation sequence in obtained in two steps. In the first step, we use the choice of $x_{i, t}$ and Lemma~\ref{lemma:concentration_bound} to bound $|f_i(x_i^*) - f(x_{i,t})|$ in terms of the posterior standard deviation at $x_i^*$ and $x_{i,t}$. 
% It is notable that, in this analysis, since $x_{i, t}$ in the exploration sequence of FLEX are selected in a purely exploratory way, we can use Lemma~\ref{lemma:concentration_bound} which provides tighter confidence intervals compared to the ones used in the analysis of GP-UCB and GP-TS~\citep{Chowdhury2017}. That is the key in proving an always sublinear regret bound for FLEX. See also~\cite{vakili2021optimal} for further discussions on the confidence intervals.
% In the second step, we show that the point selection rule in the exploration sequence, based on maximally reducing the uncertainty, allows us to bound both of the posterior standard deviation terms mentioned above by $\sqrt{\gamma_{N_t}/N_t}$, up to an absolute constant factor. We arrive at the theorem by summing the instantaneous regret over $i$ and $t$. A detailed proof is provided in the supplementary material.


% The proof of the theorem consists of two main steps. In the first step, we use the choice the  of $x_{i, t}$ Lemma~\ref{lemma:concentration_bound} to bound the error $|f_i(x) - \mu_{t-1}^{f_i}(x)|$. We would like to emphasize that since FLEX computes the posterior mean and variance only based on points queried in the exploration sequence, which are independent of exogenous noise, we can invoke Lemma~\ref{lemma:concentration_bound} for obtaining tighter concentration bounds here instead of the standard self-normalized concentration inequality as used in~\cite{Chowdhury2017} which results in looser upper bounds.
% This results in an upper bound in the form of 


% Firstly, we show that $|f_i(x) - \mu_{t-1}^{(i)}(x)| \leq \beta_i(\delta) \sigma_{t-1}^{(i)}(x)$ holds for all $t \geq 1$ with probability $\delta$. This results largely follows from~\cite{} and is similar to the self-normalized concentration inequality established in~\cite{Chowdhury2017}. The primary difference here is to use the fact that the points chosen in the exploration sequence are independent of the noise sequence resulting in better concentration bounds and consequently tighter regret guarantees. In the second step the above relation is used to show that regret incurred during the exploitation sequence can be bounded using the sum of posterior variances which can then be related to the information gain term. On the other the regret incurred during the exploration sequence is simply bounded using the length of the sequence. On combining these two terms, we arrive at the final bound. The detailed proof can be found in the supplementary material.

==> arXiV version copy/Introduction.tex <==
\section{Introduction}

 \subsection{Kernel-based Bandit Problems}
We consider zeroth-order stochastic optimization where the objective function is unknown but assumed to live in a Reproducing Kernel Hilbert Space (RKHS) associated with a known kernel. A learner sequentially chooses points to query and receives noisy feedback on the function values at the query points. The goal is to converge quickly to the optimizer of the underlying unknown function. A typical application is learning a classifier or predictor 
based on random instances (e.g., text prediction based on past typing instances). The stochastic objective function is the \emph{expected} reward representing the performance of the predictors. The objective function is unknown due to the unknown probabilistic model of the dependency of the next word on the past. The learner can try a predictor (i.e., the current query point) on the current instance and observes the associated reward, which is a random realization of the objective function value at the queried point.  \\

The above zeroth-order stochastic optimization problem can be equivalently viewed as a continuum-armed kernelized-bandit problem~\citep{Kanagawa2018}. The RKHS model allows for a greater expressive power for representing a broad family of objective functions. In particular, it is known that the RKHS of typical kernels, such as Mat\'ern family of kernels, can approximate almost all continuous functions on compact subsets of $\R^d$~\citep{Srinivas2010}.
Under a centralized setting where all data is available at a single decision maker, several algorithms have been proposed, including  UCB-based algorithms~\citep{Srinivas2010, Chowdhury2017}, batched pure exploration~\citep{li2022gaussian}, and tree-based domain shrinking~\citep{Salgia2020GPThreDS}. \\


In many applications, we encounter stochastic optimization in a distributed setting with multiple clients. For example, in a federated learning setting of the text prediction problem, multiple mobile users aim to learn a text predictor by leveraging each other's local data but without sharing their raw data~\citep{Li2020Survey}. Another example, more specific to the kernelized bandit setting, is hyperparameter tuning in federated learning~\citep{Dai2020FBO}. Due to the large expressive power of RKHS functions, hyperparameter tuning in centralized settings is often carried out by modelling the accuracy of the underlying neural network as an unknown function of the hyperparameters and belonging to an RKHS.
% hyperparameter tuning is carried out using Bayesian optimization which shares its algorithmic toolbox with optimization of functions in RKHS. \blue{(This sentence is not clear. What is "which" referring to"? Who is "its"? What is "algorithmic toolbox", and what is the "optimization" that is sharing the algorithmic toolbox? It would be good to explain the problem at a high level without using terminologies only people familiar with the specific problems can understand. The same with "its" in the next sentence.}
However, when a model is being learned by a collective effort of multiple clients, the hyperparameters of the model often also need to be tuned collaboratively using the information from all clients, resulting in a distributed stochastic optimization problem of a RKHS function. An interesting application of distributed optimization of RKHS functions is in the analysis of the collaborative training of neural nets using the recent theory of Neural Tangent Kernel~\citep{jacot2018neural}. \\



% .... (move all other examples such as hyperparameter tuning in federated learning~\cite{Dai2020FBO} that motivating the distributed setting here. Just talk about the examples at the high level to connect with the description of stochastic optimization in the first paragraph, similar to the text prediction example.)

% Furthermore, it lends itself to various real-world applications such as hyperparameter tuning in federated learning~\cite{Dai2020FBO}. In centralized setups, hyperparameter tuning is carried out using Bayesian optimization which shares its algorithmic toolbox with optimization of functions in RKHS.
% Developing algorithms for kernel-based optimization can help design efficient algorithms for tuning hyperparameters when the model is being learned under a distributed setting. Another application is in the collaborative training of neural nets using the recent theory of Neural Tangent Kernel~\cite{jacot2018neural}.

Comparing with the centralized setting, distributed stochastic optimization gives rise to two new challenges. First, the probabilistic model underlying local data generation may be different across clients, resulting in different local objective functions and hence the pursuit of different optimizers at distributed clients. Consider for example the text prediction problem. The probabilistic dependency of the next word on the past typed words may exhibit discrepancies caused by  geographical or cultural differences across users. This drift in data distribution calls for learning algorithms that strike a balance between data sharing and targeted local performance. In particular, how heterogeneous clients can learn collectively by leveraging each other's data while at the same time converging to an optimizer that takes into account each client's local data model. 
The prevailing approach where all clients aim to optimize a common global objective function given by a weighted sum of each client's local objectives with prefixed weight operates at one extreme of the spectrum by focusing solely on reaping the benefit of data sharing while ignoring each client's local performance.  
%The first of these is the stochastic heterogeneity across clients. In distributed settings, the popular approach where all clients work towards optimizing a common, global objective function falls short in scenarios where the data distribution is different across clients, i.e., the clients are statistically heterogeneous~\cite{Kairouz2021}. Consider, for example, the task of learning a model for predictive text in cellphones, where one would intuitively expect better accuracy as more devices participate in learning thereby giving access to more information. However, this intuition does not translate well into practice. The aberration can be attributed to the changes in data distribution influenced by geographical and cultural aspects as this variation negates the benefits of having access to more data. 
The second challenge is the communication overhead associated with information exchange across clients. While communication is necessary for collaborative learning, low communication cost is of practical importance in many applications.
%to ensure practical feasibility of algorithms. For example, when the participating devices are cellphones, a high communication cost imposes the participating devices, i.e., cellphones, to be connected to a high bandwidth network which is often difficult to ensure in practice. 
% First, (talk about stochastic heterogeneity across clients. connect with the motivating examples). Second, communication overhead.  (the writing of the challenge here can be more at high level. You can then move quickly to the next section on the formulation and contribution of this work. We can treat the formulation using personalization as an approach to deal with heterogeneity, hence a contribution itself.) 
These challenges have not been adequately addressed in the literature, especially within the kernel-based distributed bandit framework (see Sec.~\ref{sub:related_work} for a detailed discussion of related work).  \\


% Addressing these issue in collaborative learning under different settings is an active area of research~\cite{Kairouz2021}. 


\subsection{Main Contributions}

Consider a distributed setting with $K$ clients connected to a central server that facilitates information exchange, a de facto setting for training large-scale machine learning models. Each client can sequentially query its local objective function (i.e., the expected reward with respect to its local data model) and observe an unbiased noisy estimate of the function value at the chosen query point. To handle heterogeneity in local data models, we adopt the personalization framework, wherein the objective of each client is to learn a mixture of their local function and the global function, where the global objective function is an average of all local functions. The personalization framework strikes a balance between the generalization capabilities of the global function and targeted local learning tailored towards each client's local model. By allowing the full range of the mixture weights (i.e., the personalization parameters), we address the full spectrum in terms of the balance between data sharing and targeted local performance.   \\

%where each of them can sequentially query points in a given domain and observe a noisy evaluation of an unknown function at the query point. All the clients are  among them. Such distributed learning settings, also referred to as collaborative learning, have become ubiquitous in the recent years and are the  today. 
%We consider the kernelized bandit problem within the collaborative learning framework, where the clients are stochastically heterogeneous and as a result, observe values of potentially different functions, referred to as \emph{local observation} functions. To tackle the issue of heterogeneity, we adopt the personalization framework, wherein the objective of each client is to learn a mixture of their local function and the global function, i.e., average of all local functions. The personalization framework allows each client to trade-off between the generalization capabilities of the global function and fitting the model to local data.


Within this personalization framework, each client is interested in maximizing its own \emph{personalized objective function}, which differs from those of other clients. The challenge here is that the personalized objectives ${f}_k$ at each user $k$ involves other users' local functions $\{h_j\}_{j\neq k}$ which cannot be observed by user $k$. In other words, the local observations at each end user $k$ provide only a partial view of the personalized objective ${f}_k$ it aims to optimize. This necessitates collaborative learning across users in order to achieve a sublinear regret order. The required user collaboration has two aspects: information sharing and collaborative exploration. Given that $h_j$ can only be queried at user $j$, it is easy to see that information sharing is necessary for each user $k$ to learn its personalized objective ${f}_k$. The need for collaborative exploration is a more nuanced and complex issue. Consider the extreme case where every user's local observations are made available to all other users. If user $k$ simply uses a centralized learning algorithm to optimize its own personalized objective function ${f}_k$, its local model may concentrate too quickly 
around its own optimal point, resulting in insufficient exploration of $h_k$ around optimal points of the personalized local models of other users, especially for a user whose optimal point is far away from that of user $k$. More specifically, even though each user aims to converge to different optimal models, collaborative exploration--in addition to information sharing---is necessary due to the coupling across users' personalized objective functions. This adds another layer of nuance to the exploration-exploitation trade-off as the exploration at every user needs to serve the goal of greater good at the network level instead of solely being sufficient for local exploitation.  \\
% \red{(I copied this from a project report I wrote. Please edit to make termilogoes and notations consistent. You can choose to not introduce notations for the functions and the optimizers here if using words suffices. I do suggest to change "local observation function" to "local objective function" or simply "local function", which seems to be more natural following the writing in the intro. But you can decide whether there is another way to make the exposition between the intro and the rest of the paper consistent.}



%any learning algorithm needs to not only address the classical exploration-exploitation trade-off for the personalized objective of all clients but also ensure effective collaboration and information exchange towards the collaborative goal of learning the global function. Specifically, the challenge for each client is to strike a balance between taking altruistic actions to contribute towards learning the global function and maximizing their individual rewards. 


We propose a new learning algorithm for kernelized distributed bandits with probabilistically heterogeneous clients. Referred to as Collaborative Exploration with Personalized Exploitation (CEPE), this algorithm is built on the key structure of interleaving exploration epochs for the collaborative learning of the global function with exploitation epochs aiming to maximize individual local performance. %Specifically, the learning horizon is partitioned into interleaving exploration and exploitation epochs of growing lengths. 
This interleaving exploration-exploitation structure not only addresses the trade-off between of data leveraging and targeted local performance, but also effectively controls the information exchange across clients for communication efficiency through a tandem design of the accompanying communication protocol. The lengths of the exploration and exploitation epochs are carefully controlled to balance learning efficiency and communication overhead associated with information exchange. \\


We analyze the performance of the proposed algorithm and show that its regret is of $\tilde{\cO}(KT^{\frac{2}{3- \kappa}})$\footnote{$\tilde{\cO}(\cdot)$ hides the polylogarthmic factors.} and its overall communication cost is of $\cO(T^{\frac{2}{3- \kappa}})$, where $\kappa \in (0,1]$ is a parameter that depends on the smoothness of the kernel.  We further establish a lower bound on achievable regret within the kernel-based collaborative learning framework for the class of Squared Exponential and Matern kernels, which are arguably the most widely used kernels in practice. The regret lower bound matches the order of the regret incurred by CEPE up to a poly-logarithmic factor, establishing the optimality of the proposed algorithm. Empirical studies demonstrate the effectiveness of the CEPE against several baseline algorithms, bolstering our theoretical results. \\

To further reduce the communication cost, we propose a variant of CEPE which employs sparse approximations of the surrogate Gaussian Process modelling used in the query and update rules of CEPE. Referred to as S-CEPE, this algorithm reduces the communication cost to $\cO(T^{\frac{2\kappa}{3- \kappa}})$ while preserving the regret guarantee of CEPE. Numerical examples demonstrate effectiveness of S-CEPE in practice as S-CEPE is shown to offer a $14$-fold reduction in communication cost while sacrificing regret by a factor of less than $2$ when compared to CEPE. \\










% \blue{The logic flow of the remaining text here is unclear. It needs to be restructured after the changes to the first subsection.}

% \blue{In this subsection, you can focus on the specific problem in this paper. First describe the problem (K distributed client fercilitated by a central server; stochastically heterogeneous data resulting in different local objective functions, etc.). Then introducing personalization as an approach to collaborative learning among heterogeneous users, which is part of the problem formulation. Following the formulation, you explain the technical challenge for this specific problem formulation: the need of collaboration and information sharing, etc. Then you explain the algorithm to echo how it handles those technical challenges, the analysis of its learning efficiency and comm. efficiency. etc., then sparcification as a further approach to deal with comm. cost to conclude the contribution. The writing of the contribution in this subsection will echo the two high-level challenges of heterogeneity and comm. cost in the first subsection. } 


% \blue{(There is some disconnect in the description of the problem in this paragraph. "playing actions, receiving rewards, observation functions" are different from "query points, objective function" etc. in the first paragraph. Intro should be easy to understand even for someone outside this subject area. Some of the text below related to the general distributed setting and underlying philosophy are no longer necessary here. )}
% \red{In this paper, we consider a distributed learning setup where $K$ clients interact with the environment by playing actions from a given set and receive rewards based on an unknown observation function, possibly different across clients. All the clients are connected to a central server that facilities information exchange among them. Such distributed learning settings have become ubiquitous in the recent years and are the de facto approach for training large-scale machine learning models today. The underlying philosophy of approaching this problem is to adopt a collaborative approach to learn a common model by leveraging information from all the participating clients. Specifically, given a current estimate of the true model parameters, each client updates its belief about the current estimate using its local data, for example by computing a noisy estimate of gradient, and transmits the newly learnt information to the central server. At the central server, such updates are aggregated and estimate is updated and shared with all the clients. Consequently, algorithm design for distributed learning consists of two components: (i) designing which actions to play, which controls the new information that is gathered, and (ii) when and how to transmit the newly learned information, which controls the communication cost.} 

% \blue{(Most of the text in this paragraph will either be move to the first subsection for the high-level challenges or can be removed.)}
% \red{In typical distributed learning algorithms, the choice of query points for different clients is designed to efficiently optimize a common global objective function. While such an approach can be effective in certain cases, it falls short in scenarios where the data distribution is different across clients, i.e., the clients are statistically heterogeneous. Consider, for example, the task of learning a model for predictive text in cellphones. At a first glance, it might seem that having more data from a larger number of participating devices is beneficial and would likely lead to better accuracy, this intuition does not translate well for practical applications. The aberration can be attributed to the changes in data distribution influenced by geographical and cultural aspects as this variation negates the benefits of having access to more data. In particular, the drift in data distribution alters the optimizer resulting in competition between the clients instead of collaboration. As a result, when the data at different clients are statistically heterogeneous, it requires learning algorithms to strike a balance between data sharing and targeted local performance. On the other hand, communication cost is often the major bottleneck in distributed learning and is related to the second aspect of the algorithm design. Addressing these issue in collaborative learning under different settings is an active area of research~\cite{Kairouz2021}. 
% }\textcolor{green}{Should we clarify that we focus on the first problem more than the second one? If not here then some place else, say in Sec II-A-2?} \blue{(We do not need to worry about this with the current modified structure. We can leave the comm. cost as a general goal without explicitly formulating it into the problem. Just highlight the comm. efficiency of CEPE and S-CEPE in the contribution.}

% \blue{(This paragraphwill be morphed or removed based on the suggested new structure of this subsection.)}
% In such scenarios, one adopts the Collaborative Learning framework, wherein the different clients cooperate by communicating with each other. Thus by sharing and pooling information using a central server as a facilitator, the clients can together learn a \emph{global} model instead of learning a \emph{local} model only using the data available to them at an individual level. This ability to learn via cooperating makes this paradigm popular in real-world scenarios. This appealing characteristic, however, is accompanied by various hurdles in algorithm design for collaborative learning. The first and arguably the most important one is that of the associated communication overhead. Greater communication clearly results in better accuracy which comes at the cost of making the learning slower and more expensive. Another issue arises when the data at different clients are statistically heterogeneous requiring algorithms to strike a balance between data sharing and targeted local performance. Addressing these issues in collaborative learning under different settings is an active area of research~\cite{Kairouz2021}.

% \blue{(This paragraph can be incorporated in the related work section, if the message is not already there. The application of hyperparameter tuning will be moved to the first subsection.)}
% While collaborative learning has been extensively studied for first-order stochastic convex optimization, multi-armed bandits and linear bandits, it has received limited attention in the zeroth-order kernel-based setting. Collaborative learning using kernel-based methods allows one to leverage the benefits of collaboration along with those of greater expressive power offered by RKHS based modelling. Furthermore, it lends itself to various real-world applications such as hyperparameter tuning in federated learning~\cite{Dai2020FBO}. In centralized setups, hyperparameter tuning is carried out using Bayesian optimization which shares its algorithmic toolbox with optimization of functions in RKHS.
% Developing algorithms for kernel-based optimization can help design efficient algorithms for tuning hyperparameters when the model is being learned under a distributed setting. Another application is in the collaborative training of neural nets using the recent theory of Neural Tangent Kernel~\cite{jacot2018neural}.


% \blue{(This paragraph below will be morphed based on the suggested new structure of this subsection.)}
% In this work, we consider the kernelized bandit problem within the collaborative learning framework with personalization, wherein the objective of each client is to learn a mixture of the global and local model to tackle any potential statistical heterogeneity across clients. Our contribution consists of three results. First, we develop a near-optimal learning policy in the aforementioned setup and analyze its regret performance. Referred to as Collaborative Exploration with Personalized Exploitation (CEPE), this policy interleaves exploration and exploitation to not only address the usual trade-off between learning vs. earning, but also to effectively control the information exchange across clients for learning the global objective (Section~\ref{section:policy}). Second, we show that sparse approximation methods can help address the bigger challenge of communication in kernel-based collaborative setups by significantly reducing the communication cost without sacrificing the regret performance (Section~\ref{section:sparsepolicy}). Third, we derive a regret lower bound for the kernel-based collaborative learning framework (Section~\ref{section:lowerbound}) \red{for the class of Squared Exponential and Matern kernels, which are arguably the most widely used kernels in practice. The regret lower bound matches the order of the regret incurred by CEPE up to a poly-logarithmic factor, demonstrating the optimality of the proposed approach, CEPE.}





% \blue{. The regret lower bound demonstrates that CEPE is order optimal up to a poly-logarithmic factor and a $\gamma^{1/3}$ factor, where ${\gamma}$ is the maximal information gain of the kernel (representing the effective dimension of the kernel, see details in Section~\ref{section:lowerbound}).}


\subsection{Related Work}
\label{sub:related_work}

Kernel-based bandit problem in the centralized setting has been extensively studied in the literature~\citep{Chowdhury2017,Srinivas2010,Valko2013a, Hensman2013, Titsias2009, Calandriello2017, Seeger2003}. The setup considered in these studies, where all the data is available at a central server, is inherently different from the distributed setup considered in this work. Please refer to  Remark~\ref{remark:singlekernel} for additional comparison with these results. \\

%With the increasing ubiquity of distributed settings, there has been an increased interest in analyzing bandit problems under distributed setups. 
% \textcolor{blue}{Is this paragraph for work on discrete bandits? If yes, should specify that in the leading sentence to show a clear classification of existing work. Even if not all are discrete bandits, need a leading sentence to specify how these bandit studies are in a different formulation from the kernel bandits reviewed in the next paragraph.}
Various studies have considered the discrete multi-armed bandit problem and linear bandit problem in the distributed setting.
\cite{Shi2021FMAB} and~\cite{Shi2021Personalization} consider the multi-armed bandit (MAB) problem in a distributed setup with homogeneous and heterogeneous client reward distributions respectively. \cite{Li2020} considered the same problem with distributionally identical clients, with a focus on ensuring privacy.~\cite{Hillel2013} consider the pure exploration problem for multi-armed bandits connected over a network. Other representative works in the MAB setting include~\citep{Liu2010DistributedMAB, Shahrampour2017, Landgren2017, Sankararaman2019}.~\cite{Wang2019distributedBandit} proposed the DELB algorithm for the distributed linear bandit setting with focus on communication efficiency.~\cite{Dubey2020} proposed a privacy preserving algorithm for distributed linear bandits with clients connected via various network topologies. Other studies exploring linear bandits in a distributed setup include~\citep{Korda2016, Huang2021, Ghosh2021, Amani2022, Salgia2022LinearBandits}. The kernel-based bandit setting is arguably more challenging than the classical MAB or the linear bandit setting. \\

The problem of kernel-based bandits in collaborative setups has not received sufficient attention. There exist only a handful studies.~\cite{Du2021CoPEKB} considered the problem of pure exploration in kernel-based collaborative learning over a finite action set. Another work in this direction is by~\cite{Li2022KernelContextBandits} where the authors propose a communication-efficient algorithm with a communication cost of $\cO(\gamma_T^{3})$.~\cite{Dubey2020KernelBandits} consider distributed kernel bandits over a graph where they consider additional kernel based modelling to measure task similarity among the different objective functions of the clients. However, their proposed algorithm suffers from a communication cost that grows linearly with the time horizon. In this work, we consider the more challenging continuum-armed setup with a focus on minimizing cumulative regret as opposed to simple regret. Moreover, the personalization framework considered in this work is different from the other studies in kernel-based collaborative learning. Furthermore, the S-CEPE algorithm proposed in this work incurs a communication cost of $\cO(T^{\frac{2\kappa}{3- \kappa}})$, improving upon the $\cO(T^{3\kappa})$ bound obtained for the algorithm in~\cite{Li2022KernelContextBandits}. \\

The problem of distributed first-order stochastic convex optimization, often referred to as Federated Learning (FL)~\citep{mcmahan2017communication}, is yet another direction of related work that has been gaining a lot of attention in the recent times. See~\cite{abdulrahman2021survey, Kairouz2021} for a survey of recent advances. Several works in FL have also considered the personalization framework~\citep{Smith2017, Jiang2019, Wang2019, Deng2020, fallah2020personalized, Hanzely2020, Kulkarni2020, Mansour2020} as considered in this work. Despite some similarities in the setup, the zeroth-order kernel-based setup considered in this work requires very different tools and techniques for algorithm design and analysis as compared to the first-order stochastic convex optimization problem considered in FL. % , requiring very different tools and techniques
















% Federated learning (FL) aims to offer the benefit of data sharing among distributed clients without exposing local data held by each client for privacy considerations. It has seen an increasing application in IoT, edge computing, healthcare and financial sectors. 
% In FL, a central server iteratively aggregates local model updates from distributed clients to learn a global model. When local datasets across clients are statistically homogeneous, the global model, with the benefit of data sharing, offers better performance than locally trained models. When clients are statistically heterogeneous, however, the global model needs to be tailored or personalized at each individual client to strike a balance between data sharing and targeted local performance. In particular, FL with personalization has been recently introduced, where instead of learning a single global model, each client learns a mixture of the global model and its own local model to explicitly tackle heterogeneity across local datasets.   

% Most existing work on FL focuses on supervised learning with gradient based optimization algorithms such as \emph{FedAvg}~\citep{ fallah2020personalized,mcmahan2017communication}. Recently, a couple of studies considered zeroth-order (i.e., gradient free) unsupervised learning within the FL framework. For instance, \cite{Shi2021Personalization} considered the multi-armed bandit problem (with a finite number of arms) within the framework of FL with personalization. The problem was motivated by applications in cognitive radio and recommender systems.
% The finite arm assumption, however, can be restrictive.

% In this work, we consider kernel-based zeroth-order stochastic optimization within the framework of FL with personalization, where zeroth order pertains to using estimated function values in model updates as compared to using gradient estimates in first-order optimization methods. Zeroth-order stochastic optimization can be equivalently viewed as a continuum-armed bandit problem, where the continuum arms form a high-dimensional set in the Euclidean space~\citep[see, e.g.,][]{agarwal2011stochastic, vakili2019stochastic}.

% % \textcolor{red}{Move this paragraph to the problem formulation section. It is not crucial and no need to include in the intro.} We note that
% % with no structural assumption on the objective functions, the continuum armed bandit problem cannot be solved even for a single client. That being said, the kernel-based modeling is a very general approach to the problem. In fact, kernel-based models for typical kernels such as Mat{\'e}rn family of kernels can approximate almost all continuous functions~\cite{Srinivas2010}. 

 
% Our contribution consists of three results. First, we develop a near-optimal learning policy for kernel-based FL with personalization and analyze its regret performance. Referred to as FL with EXploration-exploitation sequencing (FLEX), this policy interleaves exploration and exploitation to not only address the usual tradeoff between learning vs. earning, but also to effectively control the information exchange across clients for learning the global objective (Section~\ref{section:policy}). Second, we show that the sparse approximation methods can significantly reduce the communication cost without sacrificing the regret performance (Section~\ref{section:sparsepolicy}). Third, we derive a regret lower bound for the kernel-based FL with personalization framework (Section~\ref{section:lowerbound}). The regret lower bound demonstrates that FLEX is order optimal up to a poly-logarithmic factor and a $\gamma^{\frac{1}{3}}$ factor, where ${\gamma}$ is the maximal information gain of the kernel (representing the effective dimension of the kernel, see details in Section~\ref{section:lowerbound}).


% \paragraph{Related Work:}
% % \textcolor{red}{A very good survey and most cited one is https://arxiv.org/abs/1912.04977  Suggest reference this one instead.}
%  

% Unsupervised learning (e.g., stochastic learning problems) within the FL framework is gaining increasing attention.
% \cite{Shi2021FMAB} considered the multi-armed bandit problem within the FL framework (without personalization). They derived performance bounds for a UCB based bandit policy.  \cite{Dubey2020, Li2020} considered the same problem with distributionally identical clients, with a focus on ensuring privacy. The most relevant work to ours is perhaps \cite{Shi2021Personalization} which considered multi-armed bandit problem under FL with personalization framework. All the works mentioned above consider a finite set of arms which may be too restrictive in many settings. The modeling contribution of this work is extending this setting to continuum armed bandit with infinitely many arms, where kernel-based models are used for the objective functions.  

% % However, like all the above works, they also consider a discrete setting with finitely many arms. On the contrary, in this work we consider the problem of continuum armed bandit with the rewards conforming to a kernel-based model, a setup arguably more general than the one considered in~\cite{Shi2021Personalization}.


% % Several recent works have considered this setting~\cite{Li2020, Shi2021FMAB, Shi2021Personalization, Dubey2020}. 

% % This work lies on the cusp of Federated Learning and Bandit literature, an increasingly active area of research referred to as ``Federated Bandits". Several recent works~\cite{Li2020, Shi2021FMAB, Shi2021Personalization, Dubey2020} have considered this setup, touching on several different ideas connected to this topic. Shi and Shen~\cite{Shi2021FMAB} consider only the maximization of the global objective function with a different observation models for the local clients leading to heterogeneity. Similarly,~\cite{Dubey2020, Li2020} also consider maximizing the global objective under the i.i.d. assumption for clients but with a focus on ensuring privacy. The work most closely related to this is by Shi et al.~\cite{Shi2021Personalization}, where in they also consider federated bandits with personalization. However, like all the above works, they also consider a discrete setting with finitely many arms. On the contrary, in this work we consider the problem of continuum armed bandit with the rewards conforming to a kernel-based model, a setup arguably more general than the one considered in~\cite{Shi2021Personalization}.

% % The problem of Federated Learning has received significant attention since it was first considered in~\cite{mcmahan2017communication}. Over the years, the problem has been extensively studied in detail with various modifications and generalizations. We refer the interested reader to the surveys for a more comprehensive overview of federated learning. One of such variants that is particularly relevant to this work is that of federated learning with personalization. As the name suggests, the focus here is to develop local models in addition to global one that personalize the output to their particular agents, improving the performance especially in heterogeneous settings. There is an extensive literature on federated learning with personalization~\cite{Smith2017, Jiang2019, Wang2019, Hanzely2020, Deng2020, Mansour2020, fallah2020personalized, Kulkarni2020}. However, all these works are cast as supervised learning in a federated setup as opposed to the bandit framework considered in this work.

% The kernel-based bandit problem (in a single client setting) has been considered in several works. Representative examples include ~\cite{ Chowdhury2017,Srinivas2010,Valko2013a}. See Remark~\ref{remark:singlekernel} for a comparison with these works. Other lines of work on continuum armed bandits exist relying on other regularity assumptions such as Lipschitz continuity~\citep{ bubeck2011x, kleinberg2008multi}, convexity~\citep{Agrawal2011} and unimodality~\citep{combes2020unimodal}, to name a few. We do not compare with these results due to the inherent difference in the regularity assumptions. 

% % Lastly, this work also bears resemblance with algorithms in kernelized bandits~\cite{Srinivas2010, Chowdhury2017} and distributed and multi-player bandit learning~\cite{Rosenski2016, Boursier2019, Landgren2017, Wang2019distributedBandit}. The literature in kernelized bandit largely focuses on optimizing a single function in contrast to the interactive multi-agent learning considered in this work. Similarly, the distributed and multi-player bandit learning are studied under the premise of finitely many arms typically in a decentralized framework, a clear distinction from problem addressed in this work.



==> arXiV version copy/Lower_Bound.tex <==



\section{Regret Lower Bound}\label{section:lowerbound}

In this section, we establish a lower bound on regret incurred by any algorithm for the problem of kernel-based collaborative learning with personalized rewards. In particular, in the following theorem, we show that even when there is no communication constraint, the total regret incurred by any learning algorithm as defined in~\eqref{eqn:regret_definition} is at least $\Omega(T^{2/(3 - \kappa)})$, where $\kappa$ characterizes the rate of maximal information gain and depends on the underlying kernel.

% we prove an $\Omega(T^{2/3})$ lower bound on total regret defined in~\eqref{eqn:regret_definition}, when there is no communication constraint. 

\begin{theorem}\label{Theorem:LB}
Consider the kernel-based collaborative learning with personalized rewards setting described in Section~\ref{sub:fl_personalization}, 
in an RKHS corresponding to the family of Squared Exponential (SE) and Matern (with smoothness $\nu$) kernels with no constraints on communication. Then, for all sets of personalization parameters $\{\alpha_1, \alpha_2, \dots, \alpha_K\}$, there exists a choice of observation functions $\{h_1, h_2, \dots, h_K\}$ for which, the cumulative regret of any policy $\pi$, satisfies
\begin{align*}
    \E[R_{\pi}(T)] = \begin{cases}
    \Omega(\alpha_{*} T^{\frac{2\nu + d}{3\nu + d}}) & \text{ for Matern kernels}, \\ \Omega(\alpha_{*} T^{2/3} (\log T)^{d/6}) & \text{ for SE kernel}.
    \end{cases}
\end{align*}
for sufficiently large time horizon $T$. In the above expression, $\alpha_{*} = \max_{i}(\min\{\alpha_i, 1 - \alpha_i\}) > 0$ is a constant that depends only on the personalization parameters. 
\end{theorem}
% \begin{proof}
% Please refer to the supplementary material for a detailed proof. 
% \end{proof}

Theorem~\ref{Theorem:LB} shows that the regret performance of CEPE (and S-CEPE) is order optimal up to logarithmic factors. Please refer to Appendix~\ref{proof:LB} for a detailed proof. %Appendix~\ref{proof:LB} the supplementary

% \emph{Proof Sketch}: To establish the lower bound, we consider a Federated bandit setting with a central server and two clients. The first client is interested in optimizing the global objective while the second client is interested in optimizing only its local objective. We consider an ensemble of functions from which the observation functions of the clients are chosen. The function ensemble is designed using ideas based on the results in~\cite{auer2002nonstochastic} and~\cite{scarllet} with significant modification to the design and analysis for the Federated setup considered in this work. We show that if the overall regret is desired to be sublinear, then the second client have to explore the suboptimal regions for a certain desired time horizon in order to help reduce the regret of the first client. By optimizing the expression, we show that optimal value of this time horizon is $\Theta(T^{2/3})$ which yields an overall regret of $\Omega(T^{2/3})$.  \\

% \emph{Proof Sketch}: The proof is inspired by the proof of the lower bound on the regret performance of non-stochastic bandit problem~\citep{auer2002nonstochastic}. We consider a FL with personalization setting with two clients and finitely many arms. We then consider a change of measure argument with two different reward models. It then can be shown that under at least one of the reward models the total regret defined in~\eqref{eqn:regret_definition} is at least $\Omega(T^{\frac{2}{3}})$. This proof is more involved than the one in~\citep{auer2002nonstochastic} in the sense that we need to account for the information sharing between the clients. We then show that the regret for the kernel-based model is at least as large as the finite model. Please refer to the supplementary material for a detailed proof. 


\begin{remark}
\cite{Shi2021Personalization} also conjectured a lower bound for the regret in the finite arm setting. Their lower bound is, however, different in the sense that it is a distribution-dependent lower bound. The distribution-dependent lower bounds typically are given in terms of the gaps (in the mean and KL-divergence) between the best arms and suboptimal arms. These bounds do not apply to our continuum arm setting as such gaps are always zero in case of infinite arms. We thus use a different method to prove a minimax bound on the regret. %That is a bound on minimum over policies and maximum over model ($\{g_i\}_{i=1}^K$).
%, in the sense that such distribution-dependent gaps are always zero in the case of infinite arms (modeled as continuous functions on compact domains)
\end{remark}

% Under this setup, we consider the case when the reward functions are assigned as follows. The best performing arm for client $1$ is  chosen uniformly at random among the first $M$ arms while for client $2$, the $M+1$ arm is always chosen as the optimal arm. For such a reward function distribution, we establish, in expectation, an inverse relation between the number of queries on sub-optimal arms for client $2$ and the regret incurred by client $1$. On optimizing this relation to minimize the overall cumulative regret, we arrive the lower bound. A detailed proof is provided in the supplementary material. % This idea is formally captured in Theorem~\ref{}.

% \emph{Proof Sketch}: The proof is inspired by the proof of the lower bound on the regret performance of non-stochastic bandit problem~\citep{auer2002nonstochastic}. We consider a FL with personalization setting with two clients and finitely many arms, a case arguably simpler the kernelized bandit problem. Under this setup, we consider the case when the reward functions are assigned as follows. The best performing arm for client $1$ is  chosen uniformly at random among the first $M$ arms while for client $2$, the $M+1$ arm is always chosen as the optimal arm. For such a reward function distribution, we establish, in expectation, an inverse relation between the number of queries on sub-optimal arms for client $2$ and the regret incurred by client $1$. On optimizing this relation to minimize the overall cumulative regret, we arrive the lower bound. A detailed proof is provided in the supplementary material. % This idea is formally captured in Theorem~\ref{}.


% We also establish lower bounds for learning under the federated setup considered in this work. We show that a regret of $\Omega(T^{2/3})$ is incurred by all the clients when there is no constraint on the communication cost. 





% \begin{remark}
% Theorem~\ref{Theorem:LB} shows that the regret performance of (S-)CEPE is order optimal up to logarithmic factors, and a $\gamma_T^{1/3}$ factor. For the SE kernel, the regret performance of (S-)CEPE is optimal up to logarithmic factors. 
% \end{remark}


==> arXiV version copy/Problem_Formulation.tex <==
\section{Problem Formulation and Preliminaries}
\label{sec:problem_formulation}

In this section, we present the problem formulation followed by preliminaries on Gaussian Processes (GPs), an important tool in the design of the proposed algorithm.

\subsection{Problem Formulation}
\label{sub:fl_personalization}

We consider a collaborative learning framework with a star topology consisting of a central server and $K>1$ clients. Each client $i \in \{1, 2 ,\dots, K\}$ is associated with a local \emph{observation} function, $h_i : \cX \to \R$, which it can access by querying any point $x$ in the domain $\cX \subset \R^d$ and consequently receiving a noisy evaluation $y = h_{i}(x) + \epsilon$, where $\epsilon$ is the noise term. These observation functions $h_i$ are known to live in the Reproducing Kernel Hilbert Space (RKHS) associated with a known positive definite kernel $k:\cX\times\cX\rightarrow \R$. We make the following assumptions on the observation functions and noise, commonly adopted in kernel-based learning~\citep{Srinivas2010, Chowdhury2017}.



% While clients cannot communicate with each other, they are all connected to the server, and can send and receive information to and from the server. Each client $i \in \{1, 2 ,\dots, K\}$ is associated with a local \emph{observation} function, $h_i : \cX \to \R$, where $\cX \subset \R^d$ is a convex and compact domain. At each time $t=1,2,3,\dots$, each client $i$, can query its own observation function at a point $x_{i,t} \in \cX$ of its choice, and receive a noisy evaluation $y_{i,t} = h_{i}(x_{i,t}) + \epsilon_{i, t}$ of the observation function, where $\epsilon_{i, t}$ is a zero mean noise term. 



% We next specify our regularity assumptions on the observation functions and noise, which are standard for kernel-based learning. 

\begin{assumption}\label{assumption1}
The RKHS norm of $h_i$ is bounded by a known constant $B_i$: $\|h_i\|_{H_k}\le B_i$, for each $i \in \{1,2,\dots, K\}$.
\end{assumption}

\begin{assumption}
The noise terms $\epsilon$ are assumed to be zero mean $R$-sub-Gaussian variables, i.e., $\E \left[ e^{\zeta \epsilon} \right] \leq \exp \left( \zeta^2 R^2/2 \right)$ for all $\zeta \in \R$, that are distributed independently across queries and clients. 
% In addition $\epsilon$ is assumed to be $R$-sub-Gaussian for all $t$. That is $\E \left[ e^{\zeta \epsilon_{i,t}} \right] \leq \exp \left( \zeta^2 R^2/2 \right)$, for all $i=1,2,\dots, K$, $t \in \N$ and $\zeta \in \R$.
\label{assumption:sub_gaussian}
\end{assumption}

\begin{assumption}
For each given $n \in \N$ and $f \in H_k$ with $\|f\|_{H_k} \leq B$, there exists a discretization $\cD_n$
of $\cX$ such that $|f(x) - f([x]_{\cD_n})| \leq 1/\sqrt{n}$, where $[x]_{\cD_n} = \argmin_{y \in \cD_n} \|x - y\|_2$ is the closest point in $\cD_n$ to $x$ in terms of $\ell_2$ distance and $|\cD_n| \leq C B^d n^{d/2}$, where $C$ is a constant independent of $n$ and $B$.
\label{assumption:discretization}
\end{assumption}


\subsubsection{Personalized Reward Function}

In a typical collaborative learning framework, the clients work together to optimize a common objective function, referred to as the \emph{global} reward function, which is defined as,
\begin{align}
    g(\cdot) := \frac{1}{K} \sum_{i = 1}^K h_i(\cdot).
\end{align}
For example,~\cite{Shi2021FMAB} considered the finite-armed bandit problem with the above mentioned objective. In a more general case, the weights $1/K$ can be replaced by any weight distribution over the $K$ clients. In typical collaborative learning problems, the motivation behind optimizing such a \emph{global} function is to leverage information across clients. The availability of additional data facilitated by the participation of more clients helps in learning a better model that generalizes well. In the context of this work, the argument of $g$ corresponds to the parameters of the model and consequently, the maximizer of $g$ corresponds to the desired optimal parameters. \\

While collaboratively optimizing $g$ can help leverage information across clients, optimizing the global objective $g$ may not always faithfully represent the interests or desires of the clients, especially in the scenario of statistically heterogeneous clients. In contrast, it can be detrimental for a client to only stick to model obtained using local data and forgo the additional generalization capabilities offered by collaboration. Following~\cite{Deng2020, Hanzely2020, Shi2021Personalization}, we consider a collaborative learning model with personalization, where each client can choose to trade-off between the generalization capabilities of the global reward function and a locally focused reward function that aims to fit local data only.
% \blue{the global objective $g$ may not be a faithful representation of the reward function of the clients, especially in the scenario of statistically heterogeneous clients. In contrast, sticking to local data for faithful representation comes at the cost of a significantly reduced accuracy in absence of collaboration. Following~\cite{Deng2020, Hanzely2020, Shi2021Personalization}, we consider a collaborative learning model with personalization, allowing the clients to trade-off between these conflicting objectives.}
In particular, we consider a personalized \emph{reward} function for each client $i$ given by,
\begin{align}
    f_i(\cdot) = \alpha_i h_i(\cdot) + (1 - \alpha_i)g(\cdot),\label{eqn:personalised_reward_function}
\end{align}
which is a linear combination of the global reward and the local observation functions. %In this setup, each client is interested in maximizing its own personalized reward function, \red{which it feels correctly represents its desire to trade-off alignment to observed local data behaviour with generalization capabilities which are necessary for future predictions}. 
Here, the personalization parameter $\alpha_i\in (0,1)$ captures the level of personalization for each client $i$. A choice of $\alpha_i \to 0$ corresponds to adopting a fully collaborative approach. Increasing the value of $\alpha_i$ reduces the impact of collaboration and as $\alpha_i \to 1$, the client moves towards adopting a model that solely targets local observations, forgoing all benefits of collaboration. In this work, we focus on the cases $\alpha_i \in (0,1)$\footnote{This condition can be relaxed to $\max_i \alpha_i > 0$ and $\min_i \alpha_i < 1$.} which corresponds to the scenario where clients have different objective functions and need to collaborate while having different personalized objectives. We would like to point out that this personalized setting is more challenging than the scenario where all clients collaboratively optimize a \emph{common} global objective (all $\alpha_i =0$) or all of them are interested in optimizing their local observation functions (all $\alpha_i = 1$).
% \blue{$\alpha_i= 0$ corresponds to the altruistic behavior of only contributing to the learning of global reward. Increasing the value of $\alpha_i$ reduces the impact of collaboration with $\alpha_i = 1$ corresponding to the scenario of optimizing only the local reward functions.}  
For clarity of terminology, we refer to $g$ as the global reward, $h_i$ as the local observation, and $f_i$ as the personalized reward for client $i$. 


\subsubsection{Communication Protocol and Cost}
\label{sub:communication_cost_definition}

% From the definition of personalized reward, we can see that, to achieve a sublinear regret, the clients need to share information about their local observations with each other. In particular, note that $f_i$ depends on all $g_j$, $j=1,2,\dots,K$. Client $i$ can learn $g_j$, $j\neq i$ only through the information provided by client $j$. Thus, the clients depend on each other to learn their own personalized reward. In the FL framework, sharing information among clients is allowed through the server. The communication protocol is formalized as follows. At times $1\le t_1<t_2<t_3<\dots$

Each personalized reward $f_i$ depends on the observation functions $h_j$ of other clients $j \neq i$ which are cannot be accessed by client $i$. The clients thus need to share information about their local observations with each other, in order to make learning $f_i$ feasible and incur a sublinear regret. In our setup, the clients can communicate only with central server and cannot communicate with other clients, a typical setting in networks with a star topology. At each time $t$, each client $i$ is allowed to send and receive a message to and from the server. For simplicity, we assume that all the communication is synchronized, a commonly adopted assumption in collaborative learning frameworks. We assign a unit cost to each communication of a scalar from the client to other clients through the server. 
% , and is the same as~\cite{Shi2021Personalization}

\subsubsection{The learning objective}

% A collaborative learning policy $\pi=\{\pi_{i,t}\}_{t\ge 1, \, i=1,2,\dots,K}$ specifies, for each client~$i$, which point $x_{i,t}$ to query at each time $t$ based on available information.
%$\pi=\{\pi_{i,t}:\cF_i^t\rightarrow\cX\}_{\substack{i=1,2,\dots,K\\ t=1,2,\dots}}$ 
%as a collection of mappings, from the information available to each client $i$ at time $t$ to an observation point for that client at that time. 
%The information $\cF_i^t$ consists of the previous observations of client $i$ from its local observation function, as well as some of the local observations from other clients provided to client $i$ by the server, yet to be specified. 
A collaborative learning policy $\pi=\{\pi_{i,t}\}_{t\ge 1, \, i=1,2,\dots,K}$ specifies, for each client~$i$, which point $x_{i,t}$ to query at each time $t$ based on available information. 
% (I suggest not making explicit the information used for decision making here which is actually part of the design (the algorithm design actually has two parts: how to choose $x_{i,t}$ and what information to exchange. Not sure how and whether we want to make the latter specific, given that we don't have a explicit constraint on communication cost. This leaves open the trivial solution of sharing everything and reduce the problem to a centralized one. Maybe you have ways to get around this?). It gives an impression that the problem is not fully specifies. Also, suggest not calling $x$ the observation point, especially we consider online setting where $x$ is not just for observations, but will be implemented as actions. Please check for other parts of the paper.) 
The performance of $\pi$ is measured in terms of total cumulative regret summed over all clients and over a learning horizon of length $T$. Specifically, 
\begin{align}
    R_{\pi}(T) = \sum_{i = 1}^K \sum_{t = 1}^T (f_i(x^*_i) - f_i(x_{i,t})),
    \label{eqn:regret_definition}
\end{align}
where $x_i^* = \argmax_{x \in \cX} f_i(x)$ is the optimal decision variable for client $i$'s personalized reward function $f_i$. \\
%\red{We would like to point out that the choice of defining the regret with respect to the personalized reward function $f_i$ is consistent with the objective of the client. Recall that $f_i$ was defined by the personalization parameter chosen by a client which decides their operating point on the trade-off between allegiance to local behaviour and generalization capabilities of a collaborative model.}
% The expectation is taken over any randomization in the policy and the noise distributions. 

The objective is to design a policy $\pi$ which minimizes the total cumulative regret. We provide high probability regret bounds that hold with probability at least $1 - \delta_0$ for any given $\delta_0 \in (0,1)$, a stronger performance guarantee than bounds on expected regret.


\subsection{Preliminaries on GP Models}\label{sec:GP}

In this section, we overview the GP models and some useful confidence intervals for the RKHS elements based on GP models, which are central to our policy design. \\

A Gaussian Process model, $H(x)$, $x \in \cX$ is a random process indexed on $\cX$, for which all finite subsets $\{H(x_i)\}_{i=1}^n$, $n\in\N$, have a multivariate Gaussian distribution, with mean $\mu(x)=\E[H(x)]$ and covariance $k(x, x')=\E[(H(x)-\mu(x))(H(x')-\mu(x'))]$. We assume $\mu(x)=0$, for all $x\in\cX$. When used as a prior for a data generating process under Gaussian noise, the conjugate property provides closed form expressions for the posterior mean and covariance of the GP model. In particular, given a set of observations $\cH_t=\{\bfx_t, \bfy_t\}$, where $\bfx_t = (x_1, x_2, \dots, x_t)^{\top}$, $\bfy_t = (y_1, y_2, \dots, y_t)^{\top}$, the following expressions can be derived for the posterior mean and covariance of the GP model 
\begin{align}
	\mu_t(x) & = \E \left[H(x) |\cH_t\right] = k_{\bfx_t, x}^{\top} \left( K_{\bfx_t, \bfx_t} + \lambda I_t \right)^{-1} \bfy_t \label{eq:posterior_mean} \\
	k_t(x, x') & = \E\left[(H(x) - \mu_t(x))(H(x') - \mu_t(x'))|\cH_t\right]  \nonumber \\
	& = k(x, x') - k_{\bfx_t, x}^{\top} \left( K_{\bfx_t, \bfx_t} + \lambda I_t \right)^{-1} k_{\bfx_t, x'}. \label{eq:posterior_variance}
\end{align}
In the above expressions, $k_{\bfx_t, x} = [ k(x_1, x), .., k(x_t, x) ]^{\top}$, $K_{\bfx_t, \bfx_t}$ is the $t \times t$ covariance matrix  $[k(x_i, x_j)]_{i,j = 1}^t$, $I_t$ is the $t \times t$ identity matrix and $\lambda$ is the variance of the Gaussian noise. We use $\sigma_t^2(\cdot)=k_t(\cdot,\cdot)$ to denote the posterior variance of the GP model. \\


% Following a standard approach in the literature~\citep[e.g., see,][]{Chowdhury2017, Shekhar2018, Srinivas2010}, we assume a fictitious GP prior for a function $h$ belonging to the RKHS. We use the notation $H$ to distinguish the fictitious GP model from the fixed function $h$. Specifically  
% Assuming also a fictitious Gaussian distribution for observation noise,

Following a standard approach in the literature (e.g., see ~\cite{Chowdhury2017, Shekhar2018, Srinivas2010}), we use GPs to model an unknown function $h$ belonging to the RKHS corresponding to the covariance kernel of the GP. In particular, we assume a \emph{fictitious} GP prior $H$ over the \emph{fixed}, unknown function $h$ along with \emph{fictitious} Gaussian distribution for the noise. We would like to emphasize that these assumptions are modelling techniques used as a part of algorithm and not a part of the problem setup. The reason for introducing this fictitious model is that the posterior mean and variance defined above, respectively, provide powerful tools to predict the values of $h$, and to quantify the uncertainty in the prediction. We formalize this statement in the following lemma.

\begin{lemma}[Theorem~$1$ in~\cite{vakili2021optimal}]
Under Assumptions~\ref{assumption1} and~\ref{assumption:sub_gaussian}, provided observations $\cH_t = \{\bfx_t, \bfy_t\}$ as specified above with the query points $\bfx_t$ chosen independently of the noise sequence, we have, for a fixed $x\in\cX$, with probability at least $1-\delta$,
\begin{align*}
|h(x)-\mu_t(x)| \leq \beta(B, \delta)\sigma_t(x),
\end{align*}
where $\beta(B, \delta)=B+R\sqrt{(2/\lambda)\log\left(2/\delta\right)}$.
\label{lemma:concentration_bound}
\end{lemma}
%Note that the randomness in the statement of the lemma comes only from the noise terms affecting $\mu_t$. The function $g$ as well as $\sigma_t$ are fixed by definition. 
This lemma shows that $\mu_t$ may be used to predict the value of $h$, where the error in the prediction is bounded by a factor of $\sigma_t$ with high probability. In CEPE, $\sigma_t(\cdot)$ is used to guide exploration and $\mu_t(\cdot)$ is used to guide exploitation.   \\

Furthermore, using the predictive variance we also define the maximal information gain, $\gamma_t$, which characterizes the effective dimension of the kernel. It is defined as $\gamma_t := \max_{(x_1, x_2, \dots, x_t) \in \cX^{t}} \sum_{i = 1}^{t} \sigma^2_{i - 1}(x_i)$. Bounds on $\gamma_t$ for several common kernels are known~\citep{Srinivas2012, Vakili2020infogain} and are increasing sublinear functions of $t$, i.e., $\gamma_t = \Oc(t^{\kappa})$ for $\kappa \in (0,1]$.
% In particular, for a Matern kernel with smoothness parameter $\nu$, $\kappa = d/(2\nu + d)$ and for Squared Exponential kernel, $\kappa \to 0$ as $\gamma_t = \Oc((\log T)^{d/2})$.}


% \subsubsection{Sparse Approximation of GP models}
% \textcolor{blue}{I suggest moving the sparse approximation to the later section where you need it. This is short and very terse; it is rather out of place here. It is better to have it where the reader needs it. In any case, the single subsubsection with only 1) but not follow-ups looks odd.}

% The sparse approximations of GP models are designed to approximate the posterior mean and variance obtained from the GP model, using a subset of observation points to reduce the computational cost associated with evaluating the exact expressions. Let $\bfz_t = \{z_1, z_2, \dots, z_m\} \subset \bfx_t$ be a subset of 
% % Let $\cJ$ be a subset of $\{1,2, \dots, t\}$ of size $m$. Using $\cJ$, we define $\cZ = \{x_j\}_{j \in \cJ}$ to a be set of
% the observation points, which we aim to use in approximating the posterior distribution of the GP model. These points are often referred to as the \emph{inducing points}. The Nystr{\"o}m approximations are given as follows~\cite{Wild2021}:
% \begin{align}
%     \tilde{\mu}_t (x) & = k_{\bfz_t, x}^{\top} (\lambda K_{\bfz_t, \bfz_t} +  K_{\bfz_t, \bfx_t} K_{\bfx_t, \bfz_t})^{-1} K_{\bfz_t, \bfx_t} \bfy_t  \label{eqn:approx_posterior_mean}\\
%     \tilde{\sigma}^2_t (x) & = \frac{1}{\lambda} \big( k(x, x) - k_{\bfz_t, x}^{\top}  K_{\bfz_t, \bfz_t}^{-1}  k_{\bfz_t, x} +  \nonumber \\
%     & \ \ \ \  \   k_{\bfz_t, x}^{\top}( K_{\bfz_t, \bfz_t} +  \lambda^{-1} K_{\bfz_t, \bfx_t} K_{\bfx_t, \bfz_t})^{-1} k_{\bfz_t, x}  
%     \label{eqn:approx_posterior_variance}
% \end{align}
% where $K_{\bfz_t, \bfz_t} = [k(z_i, z_j)]_{i,j = 1}^m \in \R^{m \times m}$, $K_{\bfz_t, \bfx_t} = [k(z_i, x_j)]_{i=1, j= 1}^{m,t} \in \R^{m \times t}$ and $K_{\bfx_t, \bfz_t} = K_{\bfz_t, \bfx_t}^{\top}$.

% The sparse approximations of the GP models are developed under two closely related but nonetheless separate approaches, with different terminologies. One approach is based on variational inference (often referred to as sparse variational Gaussian processes, SVGP), and one approach is based on Nystr{\"o}m method. The representative works are~\cite{Hensman2013, Titsias2009, vakili2020scalable} on the former, and~\cite{Calandriello2019, Calandriello2017, Seeger2003} on the latter. A recent overview~\citep{Wild2021} of these methods has shown that they essentially lead to the same result using the same computational steps. In this paper, we use the terminology of Nystr{\"o}m method.

% Recall the closed form expressions for the posterior mean and covariance of the GP model based on $t$ observations $\cH_t =\{(\bfx_t, \bfy_t)\} $, given in equation~\eqref{eq:posterior_mean} and~\eqref{eq:posterior_variance}. 


% \blue{Can remove the next two paragraphs.} The RKHS corresponding to $k(\cdot,\cdot)$, denoted by $H_k$, is a Hilbert space equipped with an inner product $\ip{\cdot,\cdot}_{H_k}$, satisfying the reproducing property: $\ip{h, k(\cdot, x) }_{H_k} = h(x)$, for all $h \in H_k$ and $x \in \cX$. The inner product induces the RKHS norm $\|h \|^2_{H_k} = \ip{h, h}_{H_k}$, that can be understood as a measure of the smoothness of the function $g$ with respect to the kernel $k$. A constructive definition of the RKHS and its norm can be given using Mercer's theorem~\citep[Theorems $4.49$, $4.51$]{steinwart2008support}. WLOG, we assume that $k(x,x) \leq 1$.

% We note that with no regularity assumption on the objective functions, the continuum armed bandit problem cannot be effectively solved even for a single client. That being said, the kernel-based modeling is a very general approach to the problem. It is known that the RKHS of typical kernels, such as Mat{\'e}rn family of kernels, can approximate almost all continuous functions on compact subsets of $\R^d$~\cite{Srinivas2010}. 

% We note that Assumption~\ref{assumption1} is a very general assumption. It is known that the RKHS of typical kernels, such as Mat{\'e}rn family of kernels, can approximate almost all continuous functions on compact subsets of $\R^d$~\cite{Kanagawa2018, Rasmussen2005}.  

% \begin{assumption}
% The noise terms $\epsilon_{i,t}$ are assumed to be independent across $i$ and $t$. In addition $\epsilon_{i, t}$ are assumed to be $R$-sub-Gaussian for all $t$. That is $\E \left[ e^{\zeta \epsilon_{i,t}} \right] \leq \exp \left( \zeta^2 R^2/2 \right)$, for all $i=1,2,\dots, K$, $t \in \N$ and $\zeta \in \R$.
% \label{assumption:sub_gaussian}
% \end{assumption}

% Lastly, we assume there exists a fine discretization of the domain for RKHS elements, which is a standard assumption in the literature~\cite{Srinivas2010, Chowdhury2017}.



% The existence of such a fine discretization is also a standard assumption in the literature~\cite{Srinivas2010, Chowdhury2017}.


% Each client can query its own function at any value $x \in \cX$ and observe a noisy estimate of the function at that point. In particular, if client $i$ queries a point $x \in \cX$, it will observe $y = g_i(x) + \epsilon^i$, where $\epsilon^i$ is a zero mean, $R$ sub-Gaussian noise, that is, $\E \left[ e^{\zeta \epsilon^i} \right] \leq \exp \left( \zeta^2 R^2/2 \right)$ for all $\zeta \in \R$. The noise samples are assumed to be i.i.d. across different samples for any particular client and also independent across clients.

% We assume a regularity condition on the functions $\{g_i\}_{i = 1}^K$ that is commonly adopted under kernelized learning models.
% Specifically, we assume that $g_i$ lives in a Reproducing Kernel Hilbert Space (RKHS)
% \footnote{The RKHS, denoted by $H_k$, is a Hilbert space associated with a positive definite kernel $k(\cdot, \cdot)$ and is fully specified by the kernel and vice versa. It is endowed with an inner product $\ip{\cdot}_k$ that obeys the reproducing property, i.e., $g(x) = \ip{g, k(x, \cdot)}_k$ for all $g \in H_k$. The inner product also induces a norm $\|g \|_{k} = \ip{g, g}_k$. This norm is a measure of the smoothness of the function $f$ with respect to the kernel $k$ and is finite if and only if $f \in H_k$.} 
% associated with a positive definite kernel $k: \cX \times \cX \to \R$. The RKHS norm of $g_i$ is assumed to be bounded by a known constant $B_i$, that is, $\|g_i \|_{k} \leq B_i$. 

% \subsection{FL with Personalization}
% \label{sub:fl_personalization}

% In the FL framework (without personalization), it is standard to define the global \emph{reward}\footnote{It may be referred to as \emph{objective} or \emph{loss} (in the case of minimization problems) in other contexts.} function as the average of the local observation functions
% \begin{align}
%     f_G(\cdot) = \frac{1}{K} \sum_{i = 1}^K g_i(\cdot).
% \end{align}
% For example, \cite{Shi2021FMAB} considered the finite armed bandit problem under this setting. 

% As discussed before, this framework may not effectively capture the heterogeneity between the clients. That is, the global reward may not suitably represent local observations $g_i$ of each client $i$.
% The global reward model can be seen as the most altruistic end of an spectrum, where the clients are only contributing to the global objective. The other end of this spectrum is purely greedy behavior that is when client $i$ aims at only learning its own $g_i$, without contributing to learning $f_G$. 

% Following~\cite{Deng2020, Hanzely2020, Shi2021Personalization}, we consider a FL with personalization model, trading off between these altruistic and greedy objectives. In particular, we consider a personalized \emph{reward} function
% \begin{align}
%     f_i(\cdot) = \alpha_i g_i(\cdot) + (1 - \alpha_i)f_G(\cdot),\label{eqn:personalised_reward_function}
% \end{align}
% for each client $i$.
% It is a linear combination of the global reward and the local observation. Here, the personalization parameter $\alpha_i\in[0,1]$ captures the level of personalization for each client $i$. $\alpha_i=0$ recovers the altruistic behavior of only contributing to the learning of global reward. While, $\alpha_i=1$ recovers the greedy behavior of independently learning the local observation function $g_i$. 

% We note that, using the definition of $f_G$, we can rewrite personalized reward as follows
% \begin{align*}
%     f_i(\cdot) = \left( \alpha_i +\frac{1-\alpha_i}{K} \right) g_i(\cdot) + \sum_{j=1, j\neq i}^K\frac{(1 - \alpha_i)}{K} g_j(\cdot).
% \end{align*}
% For clarity of terminology, we refer to $f_G$ as the global reward, $g_i$ as the local observation, and $f_i$ as the personalized reward for client $i$. 

% In the federated bandit model, the observed reward functions of the clients belong to a spectrum, the two ends of which are popularly referred to as the local and global bandit learning scenarios respectively. In the local model, the reward function associated with each client it is own local reward function. This represents the case when the clients function independently of each other and are interested in only using their own data. On the other hand, in the global model, all the clients share a collective objective of optimizing the global reward function $g_G$, given by the mean of all the observation functions, that is,
% \begin{align}
%     g_G = \frac{1}{K} \sum_{i = 1}^K g_i.
% \end{align}
% The global model corresponds to the case when the clients pool their data together to improve performance. 

% On the lines of the setup in~\cite{}, we consider the personalized reward that lies somewhere in between these two extremes. Specifically, each client sets a personalization parameter $\alpha_i \in  (0,1)$, ahead of time, that allows them to control the amount of personalization. This parameter $\alpha_i$, consequentl determines the reward function for client $i$ by taking a convex combination of the local and the global reward models.  In particular, the personalized reward function for client $i$ is given as
% \begin{align}
%     f_i = \alpha_i g_i + (1 - \alpha_i)g_G.\label{eqn:personalised_reward_function}
% \end{align}
% It is clear from the above expression how varying $\alpha_i$ can lead to a spectrum of reward functions for an client. At $\alpha_i = 1$, the personalized reward function reduces to the local reward function while for $\alpha_i = 0$, we arrive at the global model. Hence, by choosing the value of $\alpha_i$, an client can determine the amount of personalization they wish to see in their content.

% and consequently determines the objective function of the corresponding client.

% We consider a reward model for this kernelized bandit problem, similar to the one considered in~\cite{} for the multi-armed bandit problem to ensure personalized learning. In particular, a local reward function is associated with each function along a global reward function that is shared by all the clients. In this work, the local reward function of each client is simply the observation function $g_i$ associated with the client. The global reward function is given by the mean of the all the observation functions of the observation functions, that is,
% \begin{align}
%     g_G = \frac{1}{K} \sum_{i = 1}^K g_i.
% \end{align}

% Each client sets a personalization parameter $\alpha_i \in  (0,1)$, ahead of time, that allows to control the amount of personalization and consequently determines the objective function of the corresponding client. In particular, the personalized reward function for client $i$ is given as
% \begin{align}
%     f_i = \alpha_i g_i + (1 - \alpha_i)g_G.
% \end{align}
% As it can be seen from the above expression, $\alpha_i$ determines the level of personalization desired by that particular client. If $\alpha_1 = 1$, then the client is only interested in complete personalization and hence is only concerned with optimizing its local function. On the other extreme, if $\alpha = 0$, then the client only considers a global model and is not interested in personalized content.

% In the FL framework, we define a learning policy $\pi=\{\pi_{i,t}:\cF_i^t\rightarrow\cX\}_{\substack{i=1,2,\dots,K\\ t=1,2,\dots}}$ as sequences of mappings, from the information available to each client $i=1,2,\dots,K$ at time $t$ to an observation point, for each client. The information $\cF_i^t$ consists of the previous observations $\{(x_{i, t'}, y_{i, t'}=g_i(x_{i, t'})+\epsilon_{i,t'})\}_{t'=1}^{t-1}$ of client $i$ from its local observation function, as well as some of the local observations from other clients provided to client $i$ by the server, yet to be specified. 

% The performance of $\pi$ is measured in terms of total cumulative regret. Specifically, 
% \begin{align}
%     R_{\pi}(T) = \sum_{i = 1}^K \sum_{t = 1}^T (f_i(x^*_i) - f_i(x_{i,t})),
%     \label{eqn:regret_definition}
% \end{align}
% where $x_i^* = \argmax_{x \in \cX} f_i(x)$. 
% % The expectation is taken over any randomization in the policy and the noise distributions. 

% The objective is to design a policy $\pi$ which minimizes the total cumulative regret. We provide high probability regret bounds that hold with probability at least $1 - \delta_0$ for any given $\delta_0 \in (0,1)$, a stronger performance guarantee than bounds on expected regret.

% \subsection{Communication Protocol and Cost}
% \label{sub:communication_cost_definition}

% % From the definition of personalized reward, we can see that, to achieve a sublinear regret, the clients need to share information about their local observations with each other. In particular, note that $f_i$ depends on all $g_j$, $j=1,2,\dots,K$. Client $i$ can learn $g_j$, $j\neq i$ only through the information provided by client $j$. Thus, the clients depend on each other to learn their own personalized reward. In the FL framework, sharing information among clients is allowed through the server. The communication protocol is formalized as follows. At times $1\le t_1<t_2<t_3<\dots$

% Each personalized reward $f_i$ depends on the observation functions $g_j$ of all clients $j$. The clients thus need to share information about their local observations among each other, in order to make learning $f_i$ feasible. We here describe the communication protocol in our FL framework. The information is shared through the server. At each time $t$, each client $i$ is allowed to send some data to the server. The data is then broadcast to all other clients. For simplicity, we assume that all the communication is synchronized, that is a typical assumption in the FL framework~\cite{mcmahan2017communication}, and is the same as~\cite{Shi2021Personalization}. The shared data is in the form of the local observations of the clients $(x_{i,t},y_{i,t})$. We assign a unit cost to each communication of a single observation to other clients through the server. 


% In order to have any hope for a policy with sublinear regret, it is imperative for the clients to be able to communicate information about their local reward function to everyone. This follows by noting that the personalized reward function depends on all the functions $\{g_i\}_{i=1}^K$ while client $i$ only has access to its own local reward function $g_i$. Hence, the problem is ill-posed unless client $i$ can learn something about $g_j$ for $j \neq i$. We enable information sharing via a client-server periodic communication, a communication model inherent to federated setups. In the classical federated learning setup, in each round of communication the clients or clients can send ``local model updates'' to a central server, which then aggregates and broadcasts the updated ``global model'' to the clients. In the context of federated bandit setup, each client can send an $(x, y)$ pair, that is, a pair of a query point and its corresponding observation to the central server in every round of communication. This corresponds to the sending ``local model updates'' in the classical setup. The central server, in the same round, can then broadcast this to all the clients similar to sending the ``global model'' to the clients. We assume that all such communications are synchronized, a typical assumption in federated setups~\cite{mcmahan2017communication}, such that all the updates from time instant $t$ are available to all the clients before the next query instant $t + 1$.

% Since the communication model adopted in this work closely resembles the one in classical federated learning setup, it also inherits the share of issues in the classical setup. In particular, it is well known that communication is a major bottleneck in federated learning setups. Thus, it is equally essential to assess the performance of a learning policy in terms of the communication cost it incurs. We assign a unit cost to each round of communication, that is sending a pair $(x,y)$ from an client to the central server and broadcasting it to all clients, similar to the classical scenario. 

% From the problem setup in the previous section, it can be noted that while each individual client can only observe their local reward function $g_i$, their objective is to optimize the personalized reward function. In order to have any hope for a policy with sublinear regret, it is imperative for the clients to be able to communicate information about their local reward function to everyone so that it is possible to learn about the global reward function and consequently the individual objective functions. We assume a communication model that is usually considered in a federated learning setup and is similar to the one considered in centralized multi-player multi-armed bandit problems. In particular, in lieu of the federated setup, the clients or clients can send ``local model updates" to a central server, which then aggregates and broadcasts the updated ``global model" to the clients. In the context of our setup, each client can send an $(x, y)$ pair, that is, a pair of a query point and its corresponding observation to the central server which is then broadcasted to all the clients by the central server. We assume that all such communications are synchonized, a typical assumption in federated setups, such that all the updates from time instant $t$ are available to all the clients before the next query instant $t + 1$.

% It is well known that communication is a major bottleneck in federated learning setups and thus is equally essential to assess the performance of a learning policy in terms of the communication cost it incurs. We assume a simple model where each communication of an $(x,y)$ from an client to the central server and its broadcast to all the clients incurs a unit cost. This is a fairly general model of communication cost that assumes that the communication channel between any client and the central server is of a similar quality.

% \subsection{Preliminaries on Gaussian processes}
% \label{sub:preliminaries_on_gaussian_processes}

%% THIS IS COPIED FROM THE NEURIPS PAPER WITH SOME MINOR CHANGES. MOST OF IT ARE DEFINITIONS WHICH IS WHY I COULD NOT CHANGE A LOT.

% We model the unknown local reward functions $\{g_i\}_{i=1}^K$, and consequently the personalized reward functions, using a Gaussian Process (GP) based modelling, a common approach for kernel-based methods. Under the GP model, the unknown function $f$ is treated hypothetically as a realization of a Gaussian process over $\cX$. A Gaussian Process $\{F(x)\}_{x \in \cX}$ is fully specified by its mean function $\mu(\cdot)$ and covariance function $k(\cdot, \cdot)$. All finite samples of the process are jointly Gaussian with mean $\E[F(x_i)] = \mu(x_i)$ and covariance $\E[(F(x_i) - \mu(x_i))(F(x_j) - \mu(x_j))] = k(x_i , x_j)$ for $1 \leq i, j\leq n$ and $n \in \N$~\cite{Rasmussen2005}. The noise $\epsilon$ is also viewed as Gaussian.


% % Gaussian processes are closely related to RKHSs~\cite{Kanagawa2018}. In particular GPs provide powerful non-parametric Bayesian models over the space of functions which can be applied to RKHS elements.

% The conjugate property of Gaussian processes with Gaussian noise allows for a closed-form expression of the posterior distribution. Consider a set of observations $\cH_t = \{\bfx_t, \bfy_t\}$ where $\bfx_t = (x_1, x_2, \dots, x_t)^T$ and $\bfy_t = (y_1, y_2, \dots, y_t)^T$. Here $y_s = {g}(x_s) + \epsilon_s$ where $x_s \in \cX$ and $\epsilon_s$ are the zero-mean noise terms,
% i.i.d. over $s$ for $s \in \N$. Conditioned on the history of observations $\cH_t$, the posterior for $f$ is also a Gaussian process with mean and covariance functions given as %follows
% \begin{align}
% 	\mu_t(x) & = \E \left[G(x) |\cH_t\right] = k_{\bfx_t, x}^T \left( K_{\bfx_t, \bfx_t} + \lambda I \right)^{-1} \bfy_t \label{eq:posterior_mean} \\
% 	k_t(x, x') & = \E\left[(G(x) - \mu_t(x))(G(x') - \mu_t(x'))|\cH_t\right]  \nonumber \\
% 	& = k(x, x') - k_{\bfx_t, x}^T \left( K_{\bfx_t, \bfx_t} + \lambda I \right)^{-1} k_{\bfx_t, x'}. \label{eq:posterior_variance}
% \end{align}
% In the above expressions, $k_{\bfx_t, x} = [ k(x_1, x), \dots, k(x_t, x) ]^T$, $K_{\bfx_t, \bfx_t}$ is the $t \times t$ covariance matrix  $[k(x_i, x_j)]_{i,j = 1}^t$, $I$ is the $t \times t$ identity matrix and $\lambda$ is the variance in the fictitious Gaussian distribution assumed for the noise terms $\epsilon_s$. The posterior variance of the GP model is denoted by $\sigma^2_t(.)=k_t(.,.)$. 
% % The bottleneck associated with computing the posterior distribution lies in inverting the matrix $K_{\bfx_t, \bfX_t} + \lambda I $, a step that has an $O(t^3)$ computational complexity.

% The reason for introducing this fictitious model is that the posterior mean and variance defined above, respectively, provide powerful tools to predict the values of $g$, and the uncertainty in the prediction. We formalize this statement in the following lemma

% \begin{lemma}[Theorem in ~cite{}]
% Under Assumptions~\ref{assumption1} and~\ref{assumption2}, provided observations $\cH_t = \{\bfx_t, \bfy_t\}$ as specified above, we have, for a fixed $x\in\cX$, with probability $1-\delta$,
% \begin{eqnarray}
% g(x)-\mu_t(x) \le \beta(\delta)\sigma_t(x)
% \end{eqnarray}
% where $\beta(\delta)=B+\frac{R}{\lambda}\sqrt{2\log(\frac{1}{\delta})}$. 
% \end{lemma}

% Gaussian processes are powerful non-parametric Bayesian models for functions in RKHSs~\cite{Kanagawa2018}. In particular, the mean function of the GP regression (eqn.~\eqref{eq:posterior_mean}) lies in the RKHS with kernel $k(\cdot, \cdot)$ with high probability. %Thereby, GPs provide powerful non-parametric Bayesian models for functions in RKHS.
% We emphasize that the GP based modelling of the local reward functions $\{g_i\}_{i = 1}^K$ and the Gaussian noise assumption are internal to the learning policy. The \emph{actual} reward functions are still deterministic functions in an RKHS and the noise obeys an arbitrary $R$-sub-Gaussian distribution. 

% % We emphasize that the GP model of  $f$ and the Gaussian noise assumption are internal to the learning algorithm. The underlying objective function $f$ is an arbitrary deterministic function in an RKHS, and the noise obeys an arbitrary $R$-sub-Gaussian distribution. 



==> arXiV version copy/Sparse_Approximation_GPs.tex <==
\section{Reducing Communication Cost via Sparse Approximation}\label{section:sparsepolicy}

%In Section~\ref{section:policy}, we introduced CEPE and provided an analysis of its regret performance. Also, as discussed, the amount of communication required by CEPE is $\Oc(N_T)$ that is upper bounded by \red{$\Oc(T^{\frac{2}{3-\kappa}})$} for the optimal choice of $N_T$. 

In this section, we develop a variant of the CEPE algorithm that leverages sparse approximations of the posterior GP models to achieve significant reduction in communication cost while preserving the optimal regret performance.We begin with some preliminaries on sparse approximations of GP followed by the description of our proposed algorithm.

%\vspace{-0.8em}

% \subsection{Sparse Approximation of GP models}

% The sparse approximations of the GP models are developed under two closely related but nonetheless separate approaches, with different terminologies. One approach is based on variational inference (often referred to as sparse variational Gaussian processes, SVGP), and one approach is based on Nystr{\"o}m method. The representative works are~\cite{Hensman2013, Titsias2009, vakili2020scalable} on the former, and~\cite{Calandriello2019, Calandriello2017, Seeger2003} on the latter. A recent overview~\citep{Wild2021} of these methods has shown that they essentially lead to the same result using the same computational steps. In this paper, we use the terminology of Nystr{\"o}m method.

% Recall the closed form expressions for the posterior mean and covariance of the GP model based on $t$ observations $\cH_t =\{(\bfx_t, \bfy_t)\} $, given in equation~\eqref{eq:posterior_mean} and~\eqref{eq:posterior_variance}. Let $\bfz_t = \{z_1, z_2, \dots, z_m\} \subset \bfx_t$ be a subset of 
% % Let $\cJ$ be a subset of $\{1,2, \dots, t\}$ of size $m$. Using $\cJ$, we define $\cZ = \{x_j\}_{j \in \cJ}$ to a be set of
% the observation points, which we aim to use in approximating the posterior distribution of the GP model. These points are often referred to as the \emph{inducing points}. The Nystr{\"o}m approximations are given as follows~\citep{Wild2021}:
% \begin{align}
%     \tilde{\mu}_t (x) & = k_{\bfz_t, x}^{\top} (\lambda K_{\bfz_t, \bfz_t} +  K_{\bfz_t, \bfx_t} K_{\bfx_t, \bfz_t})^{-1} K_{\bfz_t, \bfx_t} \bfy_t  \label{eqn:approx_posterior_mean}\\
%     \tilde{\sigma}^2_t (x) & = \frac{1}{\lambda} \big( k(x, x) - k_{\bfz_t, x}^{\top}  K_{\bfz_t, \bfz_t}^{-1}  k_{\bfz_t, x} +  \nonumber \\
%     & \ \ \ \  \   k_{\bfz_t, x}^{\top}( K_{\bfz_t, \bfz_t} +  \lambda^{-1} K_{\bfz_t, \bfx_t} K_{\bfx_t, \bfz_t})^{-1} k_{\bfz_t, x}   %\nonumber 
%     \label{eqn:approx_posterior_variance}
%     % \tilde{\mu}_t (x) & = \bfz_t(x) \bfV^{-1}_t(\bfx_t) \bfZ^{\top}_t(\bfx_t) \bfy_t
%     % \tilde{\sigma}^2_t (x) & = \frac{1}{\lambda} \big( k(x, x) - \nonumber \\
%     % & \ \ \ \  \ \bfz^{\top}(x) \bfZ^{\top}(\bfx_t) \bfZ(\bfx_t) \bfV^{-1}(\bfx_t) \bfz(x) \big)
% \end{align}
% where $K_{\bfz_t, \bfz_t} = [k(z_i, z_j)]_{i,j = 1}^m \in \R^{m \times m}$, $K_{\bfz_t, \bfx_t} = [k(z_i, x_j)]_{i=1, j= 1}^{m,t} \in \R^{m \times t}$ and $K_{\bfx_t, \bfz_t} = K_{\bfz_t, \bfx_t}^{\top}$.
% where, $\bfz (x) = (K_{\cZ, \cZ}^{1/2})^{+} k_{\cZ, x}$, $\bfZ(\bfx_t)  = [\bfz(x_1), \dots, \bfz(x_t)]^{\top} $ and $\bfV(\bfx_t)  = \bfZ^{\top}(\bfx_t) \bfZ(\bfx_t) + \lambda I_m$.
% \begin{align*}
%     \bfz (\cdot) & = (K_{\cZ, \cZ}^{1/2})^{+} k_{\cZ, \cdot} \\
%     \bfZ & = [\bfz(x_1), \dots, \bfz(x_M)]^T \\
%     \bfV & = \bfZ^T \bfZ + \lambda I.
% \end{align*}
% Recall that $k_{\cZ, x}$ was defined as $|\cZ| \times 1$ vector with $k(x_j, \cdot)$ as the entries for $j \in \cJ$.
% In the expression above, the notation $A^+$ denotes the pseudo-inverse of a matrix $A$.

% Here we give explicit expressions for these approximations similar to the ones we gave for the exact models. 

% Recall the closed form expressions for the posterior mean and covariance of the GP model based on observations $\cH =\{(\bfx, \bfy\}, given in equation~\eqref{eq:posterior_mean} and~\eqref{eq:posterior_variance}. Let $\{z_i\}_{i=1}^m\subset X$ be a subsample of the observation points, which we aim to use to approximate the posterior distribution of the GP model. These points are often referred to as the \emph{inducing points}. The Nystr{\"o}m approximations are given as follows
% \begin{eqnarray}
% \bar{mu}_{t} ...\\
% \bar{k}_ ...\\
% \end{eqnarray}
% where . Here we give explicit expressions for these approximations similar to the ones we gave for the exact models. 

% Ideally, this should follow, with a lemma similar to Lemma $1$. For that however we need to specifically give the method for selecting $z_i$. 

% \subsection{Sparse CEPE}
% \label{sub:sparse_fed_ex2}

\subsection{Sparse Approximation of GP models}

The sparse approximations of GP models are designed to approximate the posterior mean and variance obtained from the GP model, using a subset of query points to reduce the computational cost associated with evaluating the exact expressions. Let $\bfz_t = \{z_1, z_2, \dots, z_m\} \subset \bfx_t$ be a subset of the query points, which we aim to use in approximating the posterior distribution of the GP model. These points are often referred to as the \emph{inducing points}. The Nystr{\"o}m approximations are given as follows~\citep{Wild2021}:
\begin{align}
    \tilde{\mu}_t (x) & = k_{\bfz_t, x}^{\top} (\lambda K_{\bfz_t, \bfz_t} +  K_{\bfz_t, \bfx_t} K_{\bfx_t, \bfz_t})^{-1} K_{\bfz_t, \bfx_t} \bfy_t  \label{eqn:approx_posterior_mean}\\
    \tilde{\sigma}^2_t (x) & = \frac{1}{\lambda} \big( k(x, x) - k_{\bfz_t, x}^{\top}  K_{\bfz_t, \bfz_t}^{-1}  k_{\bfz_t, x} +  \nonumber \\
    & \ \ \ \  \   k_{\bfz_t, x}^{\top}( K_{\bfz_t, \bfz_t} +  \lambda^{-1} K_{\bfz_t, \bfx_t} K_{\bfx_t, \bfz_t})^{-1} k_{\bfz_t, x}  
    \label{eqn:approx_posterior_variance}
\end{align}
where $K_{\bfz_t, \bfz_t} = [k(z_i, z_j)]_{i,j = 1}^m \in \R^{m \times m}$, $K_{\bfz_t, \bfx_t} = [k(z_i, x_j)]_{i=1, j= 1}^{m,t} \in \R^{m \times t}$ and $K_{\bfx_t, \bfz_t} = K_{\bfz_t, \bfx_t}^{\top}$.


\subsection{CEPE with Sparse Approximation}
\label{sub:sparse_fed_ex2}

Referred to as S-CEPE, this variant of CEPE 
%is designed with a blueprint similar to that of CEPE with some minor differences to leverage the sparse approximation of GP model in order to reduce the communication cost. Similar to Section~\ref{sec:flex_description}, we describe the design of the three components of S-CEPE, namely, the epoch structure, communication protocol and query policy, one by one. 
adopts a simpler design of interleaved exploration-exploitation phases. It consists of a single exploration phase of length $N_T$, entirely concentrated at the beginning of the time horizon, followed by an exploitation phase till the end of the time horizon. Such a design provides the clients with the entire exploration sequence which is required to construct the set of inducing points in Nystr\"om approximation.  \\

Unlike CEPE, the communication in S-CEPE is completely carried out in the exploitation phase. In particular, all the communication is carried during the first $N_T^{(c)}$ steps of the exploitation phase, which are referred to the communication phase. At the $s^{\text{th}}$ instant during this communication phase, client $i$ sends $(z_{i, s}, \bfw_{i, s})$ to the server, where $z_{i,s}$ denotes the $s^{\text{th}}$ inducing point and $\bfw_{i, s}\in \R$ denotes the $s^{\text{th}}$ element of the vector $\bfw_i$. The construction of the inducing points and the vector $\bfw_i$ is described below. The server then broadcasts this to all the clients. The length of the communication sequence, $N_T^{(c)}$, is set to $9(1 + 1/\lambda) q_0 \gamma_{N_T}$ to allow all clients to complete their communication with high probability (See Lemma~\ref{lemma:inducing_set_size}), where $q_0$ is a constant specified later. \\

The messages communicated during S-CEPE are determined using the sparse approximation of GP models. Specifically, at the end of the exploration epoch, each client $i$ constructs its set of inducing points $\bfz_{i, N_T} = (z_{i, 1}, z_{i, 2}, \dots, z_{i, M_i})$ by including each point $x_{i,j} \in \bfx_{i,N_T}$ queried during the exploration epoch with a probability equal to $q_0 \left[\sigma^{(h_i)}_{N_T}(x_{i,j})\right]^2$, independent of other points. Here $q_0$ is a constant that is used to appropriately scale the probabilities of inclusion to ensure a sufficiently large set for a good approximation~\citep{Calandriello2019} and $M_i$ denotes the random cardinality of the set of inducing points of client $i$. Each client $i$, using their set of inducing points, then proceeds to compute the vector $\bfw_i = (\lambda K_{\bfz_{i, N_T}, \bfz_{i, N_T}} +  K_{\bfz_{i, N_T}, \bfx_{i, N_T}} K_{\bfx_{i, N_T}, \bfz_{i, N_T}})^{-1} K_{\bfz_{i, N_T}, \bfx_{i, N_T}} \bfy_{i, N_T}$.  \\
% The set of inducing points $\bfz_{i, N_T}$ along with the vector $\bfw_i$ is communicated by the clients to the server as described below.

The query policy used for S-CEPE during the exploration phase is same as that for CEPE, that is, to query points based on maximum uncertainty. During the exploitation phase of S-CEPE, each client $i$ chooses to query the maximizer of the predictive mean of their \emph{local} observation function, $\argmax_{x\in\cX} \mu_{N_T}^{(h_i)}(x)$ for the communication phase. After the communication phase, the clients query the maximizer of the Nystr\"om approximate posterior mean of their personalized reward function for the rest of the epoch. The approximate posterior mean of $f_i$ is given as
$$\tilde{\mu}_{N_T}^{(f_i)}(\cdot) = \alpha_i \tilde{\mu}_{N_T}^{(h_i)}(\cdot) + \frac{(1 - \alpha_i)}{K} \sum_{j = 1}^K \tilde{\mu}_{N_T}^{(h_j)}(\cdot)$$ with $\tilde{\mu}_{N_T}^{(h_i)}$'s as defined in~\eqref{eqn:approx_posterior_mean}. 
% Due to space constraints, we provide a pseudocode for S-CEPE in the supplementary material.
A pseudocode for S-CEPE is provided in Algorithm~\ref{alg:sparse_fed_exp2}.
 
\subsection{Performance Analysis}

We first establish a bound on the length of the communication sequence. The following lemma, which is a slightly modified version of Theorem~$1$ in~\cite{Calandriello2019}, gives us an upper bound on the largest inducing set among all the clients.

\begin{lemma}\label{lemma:inducing_set_size}
Fix $\delta \in (0,1)$, $\varepsilon \in (0, 1)$ and let $\chi = \frac{1 + \varepsilon}{1- \varepsilon}$. If the set of inducing points is constructed as outlined in Section~\ref{sub:sparse_fed_ex2} with $q_0 \geq 6\chi \log(4TK/\delta)/\varepsilon^2$, then with probability at least $1 - \delta$, $\max_{i} M_i \leq 9(1 + 1/\lambda) q_0 \gamma_{N_T}$.
\end{lemma}
We can conclude from the above lemma that choice of $N_T^{(c)}$ used in S-CEPE allows for sufficient time for all the clients to transmit their messages to the server in the communication phase. As a result, the communication cost of S-CEPE can be bounded by $N_T^{(c)} = \cO(\gamma_{N_T}) = \cO(N_T^{\kappa})$. The communication cost of S-CEPE is significantly lower than that of CEPE. For example in the case of SE kernel with the optimal choice of $N_T = \cO(KT^{\frac{2}{3}}(\log({T/\delta_0}))^{(d+2)/6})$, the communication cost of S-CEPE is bounded by $\Oc(K\log^{d+1}(T))$, while the communication cost of CEPE is in $\cO(KT^{\frac{2}{3}}(\log({T/\delta_0}))^{(d+2)/6})$. Furthermore, S-CEPE achieves this significant reduction in communication cost while maintaining the regret guarantees of CEPE, as shown in the following theorem.

\begin{theorem}
Consider the kernel-based collaborative learning with personalized rewards as described in Section~\ref{sub:fl_personalization}.
%
Under Assumptions~\ref{assumption1} and~\ref{assumption:sub_gaussian}, the regret performance of S-CEPE satisfies
% If S-CEPE based on Nystr\"om approximation as described in Algorithm~\ref{alg:sparse_fed_exp2} is run under this setup, then with probability at least $1-\delta_0$ for $\delta_0\in(0,1)$, the regret of SFLEX Satisfies 
\begin{align*}
R_{\text{S-CEPE}}(T) = \cO\left( K N_T + K T\sqrt{\frac{\gamma_{N_T}}{N_T} \log \left( T/\delta_0  \right)} \right).
\end{align*}
with probability at least $1-\delta_0$ for any $\delta_0 \in (0,1)$. 
% In addition, the communication cost of S-CEPE is bounded by $N_T^{(c)} =  \Oc(\gamma_{N_T}) = \cO(N_T^{\kappa})$. 
\label{thm:sparse_fed_exp2}
\end{theorem}

\begin{proof}
The proof of this theorem is similar to that of Theorem~\ref{thm:regret_fed_exp} and we provide a sketch of the proof below. We bound the regret in exploration, communication and the exploitation phases separately. The regret during the exploration phase and the communication phase is bounded within a constant factor of their length, i.e., $\cO(KN_T)$ and $\cO(K\gamma_{N_T})$ respectively.
% The exploration regret is bounded by $\Oc(KN_T)$. The regret in communication regret is similarly bounded based on the length of the communication sequence: $\Oc(K\gamma_T)$. 
The exploitation regret is bounded following similar steps as in the proof of~\ref{thm:regret_fed_exp}, except that we bound the instantaneous regret based on approximate posterior standard deviation in contrast to the exact one using Lemma~\ref{lemma:concentration_bound_sparse}, described below. 
\end{proof}

% To do this, we use 
The following lemma is a counterpart to Lemma~\ref{lemma:concentration_bound}, in the case of sparse approximation of the posterior mean and variance.


% The proof of the theorem is similar to that of Theorem~\ref{thm:regret_fed_exp}. The regret incurred during the exploration, communication and the exploitation sequences is considered separately. The regret during the exploration and communication sequence is bounded within a constant factor of their length. For the points in the exploitation sequence, $f(x_{i}^*)$ and $f(x_{i,t})$ are bounded within a constant factor of the \emph{approximate} posterior standard deviation using the following lemma, which is an equivalent of Lemma~\ref{lemma:concentration_bound}, for sparse approximation of the posterior mean and variance.

\begin{algorithm}[!h]
	\caption{S-CEPE}
	\label{alg:sparse_fed_exp2}
	\begin{algorithmic}
		\STATE {\bfseries Input:} $N_T$, the kernel $k(\cdot, \cdot)$, $\varepsilon \in (0, 1)$, $\delta_0 \in (0,1)$, $\lambda$.
		\STATE $\bfz_{i, N_T} \leftarrow \{ \}$, $q_0 \leftarrow 6(1 + \varepsilon) \log(8TK/\delta_0)/\varepsilon^2(1 - \varepsilon)$,
		$N_T^{(c)} \leftarrow 9(1 + 1/\lambda) q_0 \gamma_{N_T}$
		\FOR{$t = 1,2, \dots, N_T$}
		\STATE Choose $x_{i,t} = \argmax_{x \in \cX} \sigma_{t-1}^{(h_i)}(x)$
		\STATE Query the function $h_i$ at $x_{i,t}$ to obtain $y_{i,t}$
		\ENDFOR
		\FOR{$j = 1,2, \dots, N_T$}
		% \STATE Set $p_j \leftarrow q_0 \left[\sigma^{(g_i)}_{N_T}(x_{i, j})\right]^2$
		\STATE Draw $W_j \sim \text{Bern}(p_j)$, where $p_j := q_0 [\sigma^{(h_i)}_{N_T}(x_{i, j})]^2$
		\IF{$W_j = 1$}
		\STATE $\bfz_{i, N_T} \leftarrow \bfz_{i, N_T} \cup \{ x_{i, j} \}$
		\ENDIF
		\ENDFOR
% 		\STATE Compute $\bfZ_{i, N_T}^{\top}(\bfx_{N_T})$ using the set of inducing points $\cZ_i$
		\STATE Evaluate the vector $\bfw_i = (\lambda K_{\bfz_{i, N_T}, \bfz_{i, N_T}} +  K_{\bfz_{i, N_T}, \bfx_{i, N_T}} K_{\bfx_{i, N_T}, \bfz_{i, N_T}})^{-1} K_{\bfz_{i, N_T}, \bfx_{i, N_T}} \bfy_{i, N_T}$
		\FOR{$s = 1, 2, \dots, N_T^{(c)}$}
		\STATE $t \leftarrow t + 1$
		\STATE $x_{i, t} \leftarrow \argmax_{x \in \cX} {\mu}_{N_T}^{(h_i)}(x)$
		\IF{$s \leq m_i$}
		\STATE Send $(z_{i, s} , \bfw_{i, s})$ to the server which is then broadcast to all clients
		\ENDIF
		\ENDFOR
		\REPEAT 
		\STATE $t \leftarrow t + 1$
		\STATE  $x_{i, t} \leftarrow \argmax_{x \in \cX} \tilde{\mu}_{N_T}^{(f_i)}(x)$ 
		\UNTIL{$t = T$}
	\end{algorithmic}
\end{algorithm}




\begin{lemma}
Under Assumptions~\ref{assumption1} and~\ref{assumption:sub_gaussian}, provided a set of observations $\cH_t = \{\bfx_t, \bfy_t\}$, with $\bfx_t$ chosen independently of the associated noise sequence, and corresponding subset of inducing points $\bfz_t$ obtained as outlined in Section~\ref{sub:sparse_fed_ex2},  we have, for a fixed $x\in\cX$, with probability at least $1-\delta$,
\begin{align*}
    |h(x)-\tilde{\mu}_t(x)| \leq \tilde{\beta}(B, \delta) \tilde{\sigma}_t(x),
\end{align*}
where $\tilde{\mu}(x)$ and $\tilde{\sigma}(x)$ are as defined in~\eqref{eqn:approx_posterior_variance} and $\tilde{\beta}(B, \delta)=B\sqrt{2\lambda/(1 - \varepsilon) } + R \sqrt{2 \log ( T/\delta )}$.
\label{lemma:concentration_bound_sparse}
\end{lemma}
Detailed proofs of Theorem~\ref{thm:sparse_fed_exp2} and Lemma~\ref{lemma:concentration_bound_sparse} are provided in Appendix~\ref{proof:sparse_fed_exp2}.
% in the supplementary material. %Appendix~\ref{proof:sparse_fed_exp2}.
% Please refer to Appendix~\ref{proof:sparse_fed_exp2} for a detailed proof of Theorem~\ref{thm:sparse_fed_exp2} and the above lemma.

% \sqrt{ \frac{2\lambda}{1 - \varepsilon} } + R \sqrt{2 \log \left( \frac{1}{\delta} \right)}


% In the previous section, we discussed how **name** facilitates the trade-off between communication cost and the regret performance. Due to the particular intertwined structure of the exploration-exploitation sequences in **name**, the observations from all the sample points are needed to be shared resulting in a communication cost that is linear in length of the exploration sequence. However, if the clients were to have access to all the points and their observations beforehand, then it is possible to have the same regret guarantees with reduced communication costs. Specifically, by borrowing techniques from sparse GP literature, we can obtain similar estimates of observation functions by sharing only a specifically chosen subset of the points whose cardinality is sublinear in the length of the exploration sequence.

% This approach is mainly built on the concept of Nystr{\"o}m embeddings, a topic that has been quite extensively studied in the sparse GP literature. Given a set of observations $\cS = \{(x_j, y_j)\}_{j = 1}^N$, let $\mu_{\cS}$ and $\sigma^2_{\cS}$ denote the posterior mean and variance under the GP model obtained using the observations in $\cS$. Nystr{\"o}m embeddings allow us to efficiently approximate the posterior mean and variance, i.e., $\mu_{\cS}$ and $\sigma^2_{\cS}$ by only using a subset of points $\cI \subset \cS$. The set $\cI$ is referred to as the set of inducing points or the subset of regressors. Naturally, the quality of approximation depends on the size and the particular points that belong to $\cI$. Hence, in order to obtain a good approximation it is important to choose the set $\cI$ carefully.

% In this section, we describe **name1**, a variant of **name** that reduces the communication cost by constructing a Nystr{\"o}m embedding using a set of inducing points chosen based on a technique described in~\cite{Calandriello2019}. The exploration sequence in **name1** is carried out all at once in the beginning. Each client queries $N$ points using the maximum variance posterior sampling technique, similar to the one employed in **name**. Then based on the technique outlined in~\cite{Calandriello2019}, the client obtains a set $\cI$ of inducing points where $\|cI\|$ is of the order $O(\gamma_N)$. Only this inducing set $\cI$ is communicated to the server for broadcast. Using the values obtained from all the clients, each client can construct an approximation of their personalized reward function, the maximizer of which is then queried for the rest of the time horizon. 

% While this scheme offers reduced communication and computation costs, it is not as conforming to a federated setup as **name**. This can be primarily attributed to the difference in schedule of communication in these schemes. In **name**, each communication consists of each client sending a \emph{single} $(x,y)$ pair to the central server which is then broadcast to all the clients resulting in $O(1)$ use of each channel at such an instant. This results in a low bandwith requirement, low latency and also ensures that the communication network is never overloaded. On the other hand, all the communication in **name1** happens during a single round which results in higher bandwidth requirements and higher latencies.


% The choice of $N$ is based on the 

% It turns out that is possible to further improve the communication costs by using properties of the exploration sequence and techniques from the GP-based modelling assumed in this work. 

% Consider the exploration sequence in isolation. It can be noted that it corresponds to a sample obtained from what is popularly known in the literature as maximum posterior variance sampling scheme. An interesting property of such a sampling mechanism is that points obtained from it are quasi-uniform. Since these set of points are also used to obtain approximations of the function via posterior mean and variance, their quasi-uniform nature can be leveraged to reduce communication costs by borrowing ideas from the sparse GP literature. It has been shown that it is possible to approximate, up to a constant factor, the posterior mean and variance corresponding to a set of $N$ uniformly distributed points by the posterior mean and variance obtained from a carefully chosen subset of those points of size $O(\gamma_N)$, referred to as inducing points. This implies that instead of transmitting the entire exploration over the communication channel, it is sufficient to send only a small fraction of the sequence while ensuring similar approximation guarantees on the function. This is the principle idea underlying **name1**, a variant of **name** with reduced communication costs.


% **name1** proceeds by uniformly sampling the domain to obtain a set of $O(T^{2/3})$ points and querying the local reward functions at those points. The RLS algorithm outlined in~\cite{} is then used to obtain the set of inducing points which is then communicated to all the clients via the central server. Each client uses these set of points obtained from all the other clients to build a UCB for their objective functions, the maximizer of which is then queried for the rest of the time horizon. A pseudo code is given in~\ref{}.

% \begin{algorithm}
% 	\caption{$\pi_{DSEE-SVGP}$}
% 	\label{alg:DSEE_SVGP}
% 	\begin{algorithmic}
% 		\STATE {\bfseries Input:} $\{B_j\}_{j = 1}^{K}$, the kernel $k(\cdot, \cdot)$.
% 		\STATE Set $t \leftarrow 0$
% 		\STATE Sample $t_0 = \lceil T^{2/3} \rceil $ points at uniform from $\cX$.
% 		\STATE Apply the RLS algorithm from Musco and Musco (2017) to obtain the set of inducing points, $\cI$
% 		\STATE Communicate the values of $\{y_i\}_{i \in \cI}$ to the central server which then broadcasts all the received values to all the clients
% 		\STATE Set $t \leftarrow t_0$
% 	    \REPEAT
% 	    \STATE $t \leftarrow t + 1$
% 	    \STATE $x_t^{(i)} = \argmax_{x \in \Omega} U_{t-1}^{(i)}(x)$
% 	    \STATE Query the local reward function $g_i$ at $x_t^{(i)}$ to obtain $y_t^{(i)}$
% 	    \UNTIL{$t = T$}
% 	\end{algorithmic}
% \end{algorithm}














% Sparse FLEX is similar to FLEX with some minor differences, outlined as follows. Firstly, the exploration sequence, consisting of $N_T$ points, is entirely concentrated at the beginning of the time horizon by setting $N_t = N_T$ in FLEX. % $N_T =T^{\frac{2}{3}}(\gamma_T\log(\frac{1}{\delta_0}))^{\frac{1}{3}}$
% This design provides the clients with the entire exploration sequence which is required to construct the set of inducing points in Nystr\"om approximation. Then, each client $i$ constructs its set of inducing points $\bfz_{i, N_T} = (z_{i, 1}, z_{i, 2}, \dots, z_{i, m_i})$ by selecting each point $x_{i,j} \in \bfx_{i,N_T}$ to be included in $\bfz_{i, N_T}$ with a probability equal to $q_0 \left[\sigma^{(g_i)}_{N_T}(x_{i,j})\right]^2$ . Here $q_0$ is a constant that is used to appropriately scale the probabilities of inclusion to ensure a sufficiently large set for a good approximation~\cite{Calandriello2019}. Consequently, the set of inducing points for each client $i$ consists of a random number of points $m_i$. Each client $i$, using their set of inducing points, then proceeds to compute the vector $\bfw_i = (\lambda K_{\bfz_{i, N_T}, \bfz_{i, N_T}} +  K_{\bfz_{i, N_T}, \bfx_{i, N_T}} K_{\bfx_{i, N_T}, \bfz_{i, N_T}})^{-1} K_{\bfz_{i, N_T}, \bfx_{i, N_T}} \bfy_{i, N_T}$.

% % matrix $\bfZ_{i, N_T}(\bfx_{N_T})$ and the vector $\bfw_i = \bfZ_{i, N_T}^{\top}(\bfx_{N_T}) \bfy_{i, N_T} \in \R^{m_i}$. 

% The second difference between FLEX and Sparse FLEX is that,
% there is a communication sequence of length $N_T^{(c)}$. At the $s^{\text{th}}$ instant of this sequence, client $i$ communicates $(z_{i, s} , \bfw_{i, s})$ to the server which then broadcasts it to all the clients. Here $\bfw_{i,s}$ denotes the $s^{\text{th}}$ element of the vector $\bfw_i$. The length $N_T^{(c)}$ is chosen such that it is larger than the number of inducing points for all the clients with high probability (See Lemma~\ref{lemma:inducing_set_size}). During the communication sequence, the clients may select arbitrary points (e.g. the maximizer of the prediction of $g_i$). % based on exploratory observations).  
% % Throughout this period, client queries $x_{i, N_T}$, the last query point in the exploration sequence.
% After the communication sequence, the clients select the maximizer of the Nystr\"om approximate posterior mean of their personalized reward function for the rest of the time horizon. The approximate posterior mean of $f_i$ is given as
% $$\tilde{\mu}_{N_T}^{(f_i)}(\cdot) = \alpha_i \tilde{\mu}_{N_T}^{(g_i)}(\cdot) + \frac{(1 - \alpha_i)}{K} \sum_{j = 1}^K \tilde{\mu}_{N_T}^{(g_j)}(\cdot)$$
% with $\tilde{\mu}_{N_T}^{(g_i)}$'s as defined in~\eqref{eqn:approx_posterior_mean}. A pseudocode is provided in Algorithm~\ref{alg:sparse_fed_exp2}.





% its posterior variance times $q_0$

% = 9(1 + 1/\lambda) q_0 \gamma_{N_T}

% The Sparse FLEX is essentially similar to FLEX. We here outline the details of the differences. The first difference is that we choose $N_t = T^{\frac{2}{3}}(\gamma_T\log(\frac{1}{\delta_0}))^{\frac{1}{3}}$ which concentrates all the exploration sequence at the beginning of the time horizon. The reason is that in order to choose inducing points for Nystr{\"o}m approximation, the clients require the entire exploration sequence. Then, each client $i$ selects its set of inducing points $\cZ_i$ from the set of observations $\cH_{i,t} =\{(\bfx_{i,t}, \bfy_{i,t})\} $ in a particular way. Specifically, $\cZ_i$ is constructed by randomly sampling the $N_T$ points in the exploration sequences, where each point is selected to be in $\cZ_i$ with a probability proportional to its posterior variance.
% Our selection of inducing points is based on the method given in~\cite{Calandriello2019}, that ensures the quality of approximation.

% Using the set $\cZ_i = (z_{i, 1}, \dots, z_{i, N_T}) \subset \bfx_{i, t}$, the matrix $\bfZ_i$ and consequently the vector $\bfw_i = \bfZ_i^T \bfy_{i,t} \in \R^{N_T}$ are computed by client $i$. Then each client $i$ communicates $(z_{i, k} , \bfw_{i, k})$ over the next $N_T$ rounds for $k = 1, 2, \dots, N_T$. Here $\bfw_{i,k}$ denotes the $k^{\text{th}}$ element of the vector $\bfw_i$.
% % the vector $\bfw_i$ and its corresponding value of $x$  
% The server broadcasts these data to all clients. Once all the clients have obtained the vectors $\{\bfw_i\}_{i = 1}^K$ from all the other clients, they construct a Nystr\"om approximation of the posterior mean of their reward function using those values. For the remaining time horizon, the clients simply use the Nystr\"om approximate posterior mean of their reward function to select the maximizer of their personalized reward.
% The approximate posterior mean is given as $\tilde{\mu}^{(f_i)}(\cdot) = \alpha_i \tilde{\mu}^{(g_i)}(\cdot) + \frac{(1 - \alpha_i)}{K} \sum_{j = 1}^K \tilde{\mu}^{(g_j)}(\cdot)$ with $\tilde{\mu}^{(g_i)}$'s as defined in~\eqref{eqn:approx_posterior_mean}.
% A pseudocode is provided in Algorithm~\ref{alg:sparse_fed_exp2}. In Algorithm~\ref{alg:sparse_fed_exp2}, $q_0$ is a constant that is used to appropriately scale the probabilities of inclusion to ensure a sufficiently large set for a good approximation.

% $Z..$ and communicates them to the server over the next $|Z|$ (also $Z^Ty$ as we discussed, we need to make these absolutely clear, currently we are not talking about them) time periods. The server broadcasts these data to all clients. We can also give a pseudocode for clarity. 




% We first prove that the size of communication sequence is at most $\Oc(\gamma_{N_T})$.






==> arXiV version copy/conclusion.tex <==
\section{Conclusion}

In this work, we formulated the personalization framework for kernelized bandits that allows to tackle the problem of statistical heterogeneity in distributed learning settings. Within this framework, each client can choose to trade-off between the generalization capabilities of a global reward function and a locally focused reward function that aims to fit local data only. For this framework, we proposed a new algorithm called CEPE that achieves a regret of $\tilde{\cO}(T^{2/(3- \kappa)})$, where $\kappa$ depends on the maximal information gain corresponding to the underlying kernel. CEPE builds upon fundamental insight that in such a collaborative learning setup with personalized objective functions, each client needs to take altruistic actions in order to help everyone optimize their own objective function. We also provide a matching lower bound, establishing the order optimality of the regret incurred by CEPE. We also propose a variant of CEPE, called S-CEPE that significantly reduces the communication cost and is based on sparse approximation of GP models. An interesting follow-up direction to analyze the behaviour of neural nets in distributed learning by connecting it to the insight from this result using the concept Neural Tangent Kernel~\cite{jacot2018neural}. 

% \blue{Maybe a reference for neural tangent kernel? Also, is it necessary to capitalize here?}




==> arXiV version copy/simulations.tex <==

\section{Empirical Studies}


In this section, we corroborate our theoretical results with empirical evidence that compares the regret incurred by CEPE against several baseline algorithms and documents the reduction in communication cost offered by S-CEPE. We begin with describing the experimental setup followed by discussing the particular experiments and their results.

\subsection{Experimental Setup}
We consider a collaborative learning setup among $K = 50$ clients. The personalization parameter of each client is drawn uniformly from the interval $[0.1, 0.9]$, independent of all other clients. The observation function for each client is drawn uniformly at random from the following set of $9$ functions: $\{h: h(x_1, x_2) = \Lambda(x_1^{i}, x_2^{j}), i,j \in \{1,2,3\}\}$, where $\Lambda: [0,1]^2\to \R$ is a standard two-dimensional benchmark function for Bayesian Optimization. We vary the choice of $\Lambda$ across experiments and specify it along with the corresponding experiment. We implement all algorithms using a uniform discretization of $900$ points over the domain, $[0, 1]^2$. We use a SE kernel with lengthscale parameter $0.2$. The observations are corrupted with Gaussian noise with $\sigma^2 = 0.01$, and $\lambda$ is set to $0.01$. The results in all the experiments are obtained for a time horizon of $T = 2000$ steps by averaging over $5$ Monte Carlo runs.

\begin{figure*}[h]
\centering
\subfloat[Comparison of regret and communication cost in S-CEPE]{\label{fig:sparseflex_plot}\centering \includegraphics[scale = 0.335]{S_CEPE_compare_plot.pdf}}
~
\subfloat[Regret incurred by different algorithms]{\label{fig:comparison_plot_branin}\centering \includegraphics[scale = 0.265]{comparison_plot_branin_updated.pdf}}
~
\subfloat[Regret incurred by different algorithms]{\label{fig:comparison_plot_camel}\centering \includegraphics[scale = 0.3]{comparison_plot_camel_updated.pdf}}
~
\caption{(a) Cumulative regret of S-CEPE after $T = 2000$ steps relative to CEPE plotted against the reduction in communication offered relative to CEPE when S-CEPE is run with different sizes of inducing sets. (b, c) Cumulative regret incurred by different algorithms over $T = 2000$ steps for different objective functions ((b) Branin, (c) Function in~\cite{sobester2008engineering})}
\label{fig:plots}
\end{figure*}

\subsection{Results}
In the first experiment, we compare the regret performance of CEPE against baseline algorithms: IGP-UCB~\citep{Chowdhury2017}, GP-EI (Expected Improvement)~\citep{wang2014theoreticalGPEI} and GP-PI (Probability of Improvement)~\citep{wang2018regretGPPI}. Since these baseline algorithms are designed for the single client setting, we appropriately modify them to adapt them to the collaborative learning setup considered in this work. Specifically, for the baseline algorithms we consider the benign setting where at each time instant $t$, the entire history of all the query points and observations of each client upto time $t - 1$ is accessible by all other clients. Each client $i$ uses this history of observations upto time $t - 1$ to construct the estimate of the observation functions of other clients which in turn is used to construct the acquisition function for the query point at time instant $t$ to maximize its personalized objective function, $f_i$. The major difference here is that query points are chosen \emph{greedily} by the clients to maximize their own objective function which might make it difficult for other clients to satisfactorily estimate (and optimize) their own objective functions. Please refer to Appendix~\ref{sec:experiments} for a more detailed description of parameter settings for the different algorithms. \\

We perform this comparison for two different choices of observation functions. In the first case, the base function $\Lambda$ is set to the Branin function~\citep{Azimi2012, Picheny2013} and the overall cumulative regret incurred by different algorithms is plotted in Fig.~\ref{fig:comparison_plot_branin}. In the second case, $\Lambda$ is set to the two-dimensional extension of the benchmark function proposed in~\cite{sobester2008engineering} and overall the cumulative regret for different algorithms for this experiment is plotted in Fig.~\ref{fig:comparison_plot_camel}. As it can be seen from both the plots, the regret incurred by CEPE is lesser than that incurred by other baseline algorithms. The results are consistent with our discussion in Section~\ref{sec:flex_description} showing that baseline GP bandit algorithms do not perform well in the collaborative setting, even with communication at each round. The altruistic observations obtained during the exploration sequence in CEPE helps all the clients and contribute towards an overall lower cumulative regret. \\


In the second experiment, we study the trade-off between communication cost and regret offered by S-CEPE. In particular, we evaluate the overall cumulative regret of S-CEPE for varying sizes of the set of inducing points obtained by varying $q_0$. Recall that the number of inducing points determines the communication cost. This is compared against the regret and communication cost incurred by CEPE. For both CEPE and S-CEPE, we set $N_T = 64$ which also determines the communication cost of CEPE. The objective functions for this case are obtained by setting $\Lambda$ to the Branin function. We plot the ratio of overall cumulative regret between S-CEPE and CEPE against the ratio between the communication cost of CEPE to S-CEPE in Fig.~\ref{fig:sparseflex_plot}. As seen from the plot, S-CEPE offers upto a $14$-fold reduction in communication cost while sacrificing regret by a factor of less than $2$. This shows the efficiency of sparse approximation methods in practice. 










% We corroborate our theoretical findings with empirical evidence obtained from three sets of experiments. In the first one, we provide numerical results on the performance of CEPE for various choices of the length of exploration epoch. We empirically confirm our theoretically obtained optimal choice of $N_t$. In the second one, we study the effect of reduced communication in S-CEPE on its regret performance. We show that S-CEPE can offer a $15$-fold reduction in the communication cost without a significant increase in regret. Lastly, we compare the performance of CEPE against baseline algorithms: IGP-UCB~\cite{Chowdhury2017}, GP-EI (Expected Improvement)~\cite{wang2014theoreticalGPEI} and GP-PI (Probability of Improvement)~\cite{wang2018regretGPPI}.

% In the first two experiments , we consider a setting of $K = 4$ agents with $\alpha_i = 0.1i$, for $i = 1, 2, 3, 4$.  For each observation function, we consider a variation of the commonly used benchmark function \emph{Branin}, defined on $[0,1]^2$, denoted by $B(x_1, x_2)$. An analytical expression of the \emph{Branin} function is given in \cite{Azimi2012, Picheny2013}.
% The observation functions are chosen as $h_1(x_1, x_2) = B(x_1, x_2), \ h_2(x_1, x_2) = B(x_1, x_2^2), \ h_3(x_1, x_2) = B(x_1^2, x_2)$ and $h_4(x_1, x_2) = B(x_1^2, x_2^2)$. For the last experiment, we consider $K = 50$ with $\alpha_i$'s drawn uniformly in $[0.1, 0.9]$. For this case, each client's local observation is chosen randomly from the set $\{h: h(x_1, x_2) = B(x_1^{i}, x_2^{j}), i,j \in \{1,2,3\}\}$ which has $9$ functions. All algorithms are implemented using a uniform discretization of $1600$ points over the domain, $[0, 1]^2$. We use a SE kernel with lengthscale parameter $0.2$. The observations are corrupted with Gaussian noise with $\sigma^2 = 0.01$, and $\lambda$ is set to $0.01$. The results in all the experiments are obtained by averaging over $10$ Monte Carlo runs.

% For the first experiment, we run the CEPE algorithm for $T = 2000$ steps, with $N_t = \lceil 0.4t^{\eta}\rceil$ for $\eta \in \{1/6, 1/4, 1/3, 1/2, 2/3, 3/4, 5/6\}$. In Fig.~\ref{fig:nt_plot}, we plot the average regret for each choice of exploration sequence. Fig.~\ref{fig:nt_plot} shows that the choice of $N_T = \Oc(T^{2/3})$ results in the smallest regret, consistent with our theoretical findings. 

% In the second experiment, we evaluate the cumulative regret of S-CEPE run with $T = 1000$ and $N_T = 300$  and varying sizes of the set of inducing points obtained by varying $q_0$. Recall that the number of inducing points determines the communication cost. The vertical axis shows the ratio between the regret performance of S-CEPE to CEPE. The horizontal axis shows the ratio between the communication cost of CEPE to S-CEPE.  
% % All experiments are averaged over $10$ Monte Carlo runs.  
% Fig.~\ref{fig:sparseflex_plot} shows that S-CEPE may offer a $15$-fold reduction in communication cost while sacrificing regret by a factor of less than $1.5$. This shows the efficiency of sparse approximation methods in practice.
% % We set $N_T = 300$. $q_0$ is varied to obtain various number of inducing points.

% In the third experiment, we compare the regret performance of CEPE with standard baseline GP bandit algorithms, namely, IGP-UCB, GP-EI and GP-PI.  For these baselines, all agents optimize their own objective functions $f_i$. For IGP-UCB, we set $B = 15$ and $R^2 = \lambda = 0.01$. The margin terms in GP-EI and GP-PI are set to $0.01$. We compare these algorithms with S-CEPE run with $N_T = \lceil 0.4 T^{2/3} \rceil = 64$ over a time horizon of $T = 2000$ steps.

% Fig~\ref{fig:comparison_plot} shows the cumulative regret of each algorithm over $T= 2000$ steps. % averaged over $10$ Monte Carlo runs
% We see that although the regret of S-CEPE initially grows faster --- that corresponds to the exploration sequence ---, eventually it achieves the lowest regret. %\hspace{0.1em}
% This experiment corresponds to our discussion in Section~\ref{section:policy}, that baseline GP bandit algorithms do not perform well in the federated setting, even with communication at each round. The observations obtained during the exploration sequence in S-CEPE helps all the agents to perform better. 

% The altruistic observations gathered in CEPE helps all the agents to perform better. 






% \section{Empirical Studies}

% \begin{figure*}[]
% \centering
% \subfloat[Dependence of Regret on $N_T$]{\label{fig:nt_plot}\centering \includegraphics[scale = 0.3]{Regret_NT_plot.pdf}}
% ~
% \subfloat[Comparison of regret and communication cost in SparseFLEX]{\label{fig:sparseflex_plot}\centering \includegraphics[scale = 0.33]{comm_reduction.pdf}}
% ~
% \subfloat[Regret incurred by different algorithms]{\label{fig:comparison_plot}\centering \includegraphics[scale = 0.37]{algos_comparison.pdf}}
% ~
% \caption{(a) Cumulative regret of FLEX over $T = 1000$ steps when run with different lengths of exploration sequence averaged over $10$ Monte Carlo runs. (b) Relative increase in cumulative regret after $T = 1000$ steps plotted against the reduction in communication when SparseFLEX is run with different sizes of inducing sets. (c)  Cumulative regret incurred by different algorithms over $T = 1000$ steps averaged over $10$ Monte Carlo runs.  }
% \label{fig:plots}
% \end{figure*}

% In this section, we corroborate our theoretical findings with empirical evidence. We perform three sets of experiments. In the first one, we provide numerical results on the performance of FLEX for various choices of the length of exploration sequence. We empirically confirm our theoretically obtained optimal choice of $N_t$. In the second one, we study the effect of reduced communication in Sparse FLEX on its regret performance. We show that Sparse FLEX can offer a $15$-fold reduction in the communication cost without a significant increase in regret. Lastly, we compare the performance of FLEX against baseline algorithms: IGP-UCB~\cite{Chowdhury2017}, GP-EI (Expected Improvement)~\cite{wang2014theoreticalGPEI} and GP-PI (Probability of Improvement)~\cite{wang2018regretGPPI}.

% In all experiments, we consider a setting of $K = 4$ agents with $\alpha_i = 0.1i$, for $i = 1, 2, 3, 4$. For each observation function, we consider a variation of the commonly used benchmark function \emph{Branin}, defined on $[0,1]^2$, denoted by $B(x_1, x_2)$. An analytical expression of the \emph{Branin} function is given in \cite{Azimi2012, Picheny2013}.
% The four observation functions are set to $g_1 = B(x_1, x_2), \ g_2(x_1, x_2) = B(x_1^2, x_2), \ g_3(x_1, x_2) = B(x_1, x_2^2)$ and $g_4(x_1, x_2) = B(x_1^2, x_2^2)$. All the algorithms are implemented using a uniform discretization of $1600$ points over the domain, $[0, 1]^2$. For the SE kernel we set the lengthscale parameter $l = 0.2$. The observations are corrupted with Gaussian noise with variance $0.01$, and $\lambda$ is also set to $0.01$.

% For the first study, we run the FLEX algorithm for $T = 2000$ steps, with $N_t = \lceil 0.4t^{\eta}\rceil$ for different value of $\eta \in \{1/6, 1/4, 1/3, 1/2, 2/3, 3/4, 5/6\}$. We plot the average regret over $10$ Monte Carlo runs for each of different exploration sequences in Fig.~\ref{fig:nt_plot}. The plot clearly shows that the choice $N_T = \Oc(T^{2/3})$ results in the smallest regret, as obtained theoretically. For the second study, we evaluate the cumulative regret of SparseFLEX at the end of $T = 1000$ steps for varying sizes of the set of inducing points. We set $N_T = 300$ and decrease $q_0$ to reduce the number of inducing points and consequently the communication cost. We plot the increase in regret relative to the case when all the points are taken against reduction in communication cost, both of which are averaged over $10$ Monte Carlo runs. As it can be seen from Fig.~\ref{fig:sparseflex_plot}, when compared to FLEX, Sparse FLEX offers a $15$-fold reduction in communication while regret goes only by a small factor of $1.4$, exhibiting its relevance in practical setups.

% In the last study, we compare the proposed algorithms against several baselines like IGP-UCB, GP-EI and GP-PI.  For the baselines, all the agents are just interested in optimizing their own objective functions $f_i$ using the particular baseline algorithm. For IGP-UCB, we set $B = 15$ and $R^2 = \lambda = 0.01$. For GP-EI and GP-PI, the margin terms are set to $0.01$. We compare them against SparseFLEX that takes $40$ samples and uses all of them to perform prediction. The cumulative regret over $T= 1000$ of each algorithm averaged over $10$ Monte Carlo runs is plotted in Fig~\ref{fig:comparison_plot}. From the plot, we note that initially FLEX incurs large regret which corresponds to the exploration phase. Once the exploration has finished, the regret increases gradually. \hspace{0.1em}On the other hand for other algorithms while the initial increase is gradual, it continues to grow at a constant rate even towards the end. This can be attributed to the greedy strategy employed by other algorithms. Thus, the altruistic exploration sequence in our algorithm helps improve the regret performance in the long term.

